Reviving, reproducing, and revisiting Axelrod's second tournament

Direct reciprocity, typically studied using the Iterated Prisoner's Dilemma (IPD), is central to understanding how cooperation evolves. In the 1980s, Robert Axelrod organized two influential IPD computer tournaments, where Tit for Tat (TFT) emerged as the winner. Yet the archival record is incomplete: for the first tournament only a report survives, and for the second the submitted Fortran strategies remain but not the final tournament code. This gap raises questions about the reproducibility of these historically influential results. We recreate the second tournament by restoring the surviving Fortran implementations to compile with modern compilers and by building a Python interface that calls the original strategy functions without modification. Using the open-source Axelrod-Python library to run tournaments, we reproduce Axelrod's main findings: TFT prevails, and successful play tends to be cooperative, responsive to defection, and willing to forgive. Strategy rankings remain mostly unchanged. We then assess the robustness of the originally submitted strategies by incorporating additional strategies, and we run one of the largest IPD tournaments to date. We find that the original tournament was especially favorable to TFT and that it is difficult to dethrone TFT when the original submissions make up the majority of the field. We also observe that several lesser-known submissions perform strongly in more diverse settings and under noise. Our contributions are: (i) the first systematic reproduction of Axelrod's second tournament; (ii) a contemporary reassessment of the original results in light of new strategies and settings; and (iii) a preserved, easy-to-use implementation of the second-tournament strategies within Axelrod-Python to support future research.

==> assets/alternate_extra_strategy_tournament_winner_proportion.tex <==
\begin{tabular}{lrrrr}
\toprule
 & 1 New (N = 209) & 2 New (N = 21736) & 3 New (N = 1499784) & 4 New (N = 77238876) \\
Winner &  &  &  &  \\
\midrule
Adaptive Tit For Tat: 0.5 & NaN & 0.000092 & 0.000232 & 0.000445 \\
EugineNier: (D,) & NaN & NaN & 0.000001 & 0.000000 \\
EvolvedLookerUp2\_2\_2\textsuperscript{\textdagger} & NaN & NaN & NaN & 0.000000 \\
Firm But Fair & NaN & 0.000046 & 0.000123 & 0.001323 \\
First by Stein and Rapoport: 0.05: (D, D) & NaN & NaN & 0.000001 & 0.000000 \\
GTFT: 0.33 & NaN & NaN & 0.000020 & 0.000405 \\
Gradual & NaN & NaN & 0.000001 & 0.000002 \\
Meta Majority Long Memory: 134 players & NaN & NaN & NaN & 0.000000 \\
Meta Majority: 213 players & NaN & NaN & NaN & 0.000000 \\
Omega TFT: 3, 8 & NaN & 0.000506 & 0.001457 & 0.002576 \\
Original Gradual & NaN & 0.000046 & 0.000218 & 0.002365 \\
PSO Gambler 2\_2\_2 Noise 05\textsuperscript{\textdagger} & NaN & 0.000046 & 0.000227 & 0.000492 \\
Resurrection & NaN & 0.000092 & 0.000256 & 0.000267 \\
Soft Joss: 0.9 & NaN & 0.000092 & 0.000285 & 0.005101 \\
Spiteful Tit For Tat & NaN & NaN & 0.000049 & 0.000139 \\
ZD-GTFT-2: 0.25, 0.5 & NaN & 0.000138 & 0.000387 & 0.004531 \\
k32r & NaN & NaN & 0.000007 & 0.000789 \\
k41r & NaN & NaN & 0.000013 & 0.000000 \\
k42r & 0.148325 & 0.269415 & 0.366403 & 0.217232 \\
k44r & NaN & 0.000230 & 0.000568 & 0.004608 \\
k49r & NaN & 0.000138 & 0.000347 & 0.000231 \\
k60r & 0.004785 & 0.011180 & 0.018820 & 0.004514 \\
k75r & NaN & 0.000506 & 0.002448 & 0.000864 \\
k92r & 0.846890 & 0.717473 & 0.608137 & 0.754116 \\
\bottomrule
\end{tabular}


==> assets/alternate_single_extra_strategy_tournament_winner.tex <==
\begin{tabular}{lr}
\toprule
 & proportion \\
Winner &  \\
\midrule
k92r & 0.847 \\
k42r & 0.148 \\
k60r & 0.005 \\
\bottomrule
\end{tabular}


==> assets/axelord_python_tournament_rankings_full.tex <==
\begin{tabular}{lccccccc}
\toprule
 & \makecell[c]{Average\\Score} & \makecell[c]{Rank} & \makecell[c]{Average\\Cooperation Rate} & \makecell[c]{Original Rank} & \makecell[c]{Reproduced Average\\Cooperation Rate} & \makecell[c]{Library Rank} & \makecell[c]{Library Average\\Cooperation Rate} \\
\midrule
EvolvedLookerUp2\_2\_2\textsuperscript{\textdagger} & 2.802 & 1 & 0.756 & - & - & 1 & 0.736 \\
Evolved HMM 5\textsuperscript{\textdagger} & 2.788 & 2 & 0.751 & - & - & 2 & 0.742 \\
Omega TFT: 3, 8 & 2.786 & 3 & 0.750 & - & - & 12 & 0.725 \\
Evolved ANN 5\textsuperscript{\textdagger} & 2.784 & 4 & 0.720 & - & - & 3 & 0.713 \\
Evolved ANN\textsuperscript{\textdagger} & 2.782 & 5 & 0.739 & - & - & 5 & 0.727 \\
Evolved FSM 16\textsuperscript{\textdagger} & 2.780 & 6 & 0.731 & - & - & 4 & 0.713 \\
Evolved FSM 16 Noise 05\textsuperscript{\textdagger} & 2.776 & 7 & 0.726 & - & - & 6 & 0.717 \\
PSO Gambler 2\_2\_2\textsuperscript{\textdagger} & 2.760 & 8 & 0.702 & - & - & 7 & 0.692 \\
Original Gradual & 2.757 & 9 & 0.808 & - & - & - & - \\
PSO Gambler 2\_2\_2 Noise 05\textsuperscript{\textdagger} & 2.756 & 10 & 0.740 & - & - & 14 & 0.723 \\
PSO Gambler Mem1\textsuperscript{\textdagger} & 2.756 & 11 & 0.734 & - & - & 9 & 0.728 \\
Evolved FSM 4\textsuperscript{\textdagger} & 2.752 & 12 & 0.793 & - & - & 10 & 0.777 \\
PSO Gambler 1\_1\_1\textsuperscript{\textdagger} & 2.752 & 13 & 0.704 & - & - & 8 & 0.702 \\
Gradual & 2.746 & 14 & 0.763 & - & - & 15 & 0.793 \\
DBS: 0.75, 3, 4, 3, 5 & 2.739 & 15 & 0.750 & - & - & 11 & 0.739 \\
k42r & 2.735 & 16 & 0.820 & 3 & 0.916 & - & - \\
Winner12 & 2.733 & 17 & 0.688 & - & - & 16 & 0.682 \\
Spiteful Tit For Tat & 2.723 & 18 & 0.691 & - & - & 19 & 0.664 \\
k60r & 2.723 & 19 & 0.691 & 6 & 0.844 & - & - \\
k85r & 2.716 & 20 & 0.627 & 33 & 0.726 & - & - \\
EugineNier: (D,) & 2.713 & 21 & 0.673 & - & - & 22 & 0.645 \\
k80r & 2.706 & 22 & 0.723 & 36 & 0.809 & - & - \\
k32r & 2.704 & 23 & 0.758 & 10 & 0.873 & - & - \\
DoubleCrosser: (D, D) & 2.703 & 24 & 0.693 & - & - & 13 & 0.677 \\
k58r & 2.703 & 25 & 0.746 & 21 & 0.852 & - & - \\
k87r & 2.702 & 26 & 0.691 & 44 & 0.767 & - & - \\
k40r & 2.698 & 27 & 0.665 & 35 & 0.746 & - & - \\
k65r & 2.698 & 28 & 0.645 & 47 & 0.715 & - & - \\
Forgetful Fool Me Once: 0.05 & 2.696 & 29 & 0.750 & - & - & 20 & 0.753 \\
k49r & 2.689 & 30 & 0.813 & 4 & 0.892 & - & - \\
k56r & 2.689 & 31 & 0.793 & 38 & 0.891 & - & - \\
k59r & 2.688 & 32 & 0.793 & 40 & 0.892 & - & - \\
Revised Downing & 2.688 & 33 & 0.793 & - & - & - & - \\
Fool Me Once & 2.682 & 34 & 0.627 & - & - & 17 & 0.624 \\
k41r & 2.682 & 35 & 0.768 & 7 & 0.865 & - & - \\
k55r & 2.681 & 36 & 0.817 & 42 & 0.903 & - & - \\
First by Shubik & 2.680 & 37 & 0.740 & - & - & - & - \\
ZD-GTFT-2: 0.25, 0.5 & 2.680 & 38 & 0.867 & - & - & 50 & 0.855 \\
Soft Joss: 0.9 & 2.679 & 39 & 0.844 & - & - & 53 & 0.829 \\
BackStabber: (D, D) & 2.675 & 40 & 0.654 & - & - & 18 & 0.641 \\
MEM2 & 2.671 & 41 & 0.609 & - & - & 23 & 0.597 \\
AON2 & 2.670 & 42 & 0.684 & - & - & 21 & 0.676 \\
k81r & 2.669 & 43 & 0.704 & 43 & 0.779 & - & - \\
Meta Hunter: 6 players & 2.663 & 44 & 0.647 & - & - & 29 & 0.638 \\
NMWE Finite Memory: 79 players & 2.661 & 45 & 0.587 & - & - & - & - \\
k44r & 2.660 & 46 & 0.790 & 5 & 0.882 & - & - \\
k84r & 2.659 & 47 & 0.785 & 9 & 0.882 & - & - \\
GTFT: 0.33 & 2.658 & 48 & 0.894 & - & - & 59 & 0.886 \\
EvolvedLookerUp1\_1\_1\textsuperscript{\textdagger} & 2.658 & 49 & 0.620 & - & - & 37 & 0.615 \\
NMWE Stochastic: 67 players & 2.658 & 50 & 0.590 & - & - & - & - \\
k38r & 2.656 & 51 & 0.780 & 34 & 0.874 & - & - \\
Michaelos: (D,) & 2.655 & 52 & 0.617 & - & - & 34 & 0.601 \\
First by Stein and Rapoport: 0.05: (D, D) & 2.653 & 53 & 0.766 & - & - & - & - \\
NMWE Memory One: 36 players & 2.651 & 54 & 0.579 & - & - & - & - \\
Resurrection & 2.648 & 55 & 0.771 & - & - & 71 & 0.749 \\
Nice Meta Winner Ensemble: 213 players & 2.646 & 56 & 0.578 & - & - & - & - \\
k92r & 2.645 & 57 & 0.794 & 1 & 0.922 & - & - \\
Adaptive Tit For Tat: 0.5 & 2.645 & 58 & 0.794 & - & - & 79 & 0.773 \\
Forgiving Tit For Tat & 2.643 & 59 & 0.801 & - & - & 81 & 0.778 \\
NMWE Deterministic: 146 players & 2.638 & 60 & 0.575 & - & - & - & - \\
General Soft Grudger: n=1,d=4,c=2 & 2.638 & 61 & 0.817 & - & - & 57 & 0.811 \\
Soft Grudger & 2.637 & 62 & 0.817 & - & - & 56 & 0.811 \\
Meta Majority Long Memory: 134 players & 2.637 & 63 & 0.739 & - & - & - & - \\
Firm But Fair & 2.636 & 64 & 0.867 & - & - & 86 & 0.856 \\
Level Punisher & 2.636 & 65 & 0.734 & - & - & 44 & 0.731 \\
k68r & 2.634 & 66 & 0.859 & 12 & 0.917 & - & - \\
k86r & 2.632 & 67 & 0.745 & 28 & 0.811 & - & - \\
NMWE Long Memory: 134 players & 2.632 & 68 & 0.575 & - & - & - & - \\
Meta Majority: 213 players & 2.631 & 69 & 0.757 & - & - & - & - \\
ZD-GEN-2: 0.125, 0.5, 3 & 2.630 & 70 & 0.855 & - & - & 62 & 0.850 \\
k66r & 2.629 & 71 & 0.795 & 20 & 0.866 & - & - \\
Evolved ANN 5 Noise 05\textsuperscript{\textdagger} & 2.624 & 72 & 0.565 & - & - & 45 & 0.544 \\
Second by Eatherley & 2.624 & 73 & 0.884 & - & - & - & - \\
k46r & 2.624 & 74 & 0.884 & 14 & 0.948 & - & - \\
TF3 & 2.624 & 75 & 0.585 & - & - & 38 & 0.575 \\
Memory Decay: 0.1, 0.03, -2, 1, Tit For Tat, 15 & 2.623 & 76 & 0.756 & - & - & - & - \\
Nice Meta Winner: 213 players & 2.622 & 77 & 0.586 & - & - & - & - \\
k72r & 2.622 & 78 & 0.841 & 13 & 0.924 & - & - \\
k43r & 2.622 & 79 & 0.581 & 39 & 0.667 & - & - \\
Doubler & 2.621 & 80 & 0.821 & - & - & 88 & 0.805 \\
Meta Majority Finite Memory: 79 players & 2.619 & 81 & 0.778 & - & - & - & - \\
GrudgerAlternator & 2.619 & 82 & 0.783 & - & - & 72 & 0.779 \\
k34r & 2.618 & 83 & 0.568 & 52 & 0.652 & - & - \\
k47r & 2.611 & 84 & 0.579 & 16 & 0.723 & - & - \\
k61r & 2.606 & 85 & 0.886 & 2 & 0.954 & - & - \\
Second by Champion & 2.606 & 86 & 0.883 & - & - & - & - \\
k35r & 2.605 & 87 & 0.787 & 11 & 0.888 & - & - \\
k79r & 2.604 & 88 & 0.804 & 26 & 0.875 & - & - \\
k91r & 2.603 & 89 & 0.839 & 30 & 0.873 & - & - \\
ShortMem & 2.601 & 90 & 0.817 & - & - & 83 & 0.809 \\
Dynamic Two Tits For Tat & 2.599 & 91 & 0.838 & - & - & 95 & 0.827 \\
k64r & 2.599 & 92 & 0.796 & 17 & 0.884 & - & - \\
Adaptive Pavlov 2011 & 2.597 & 93 & 0.745 & - & - & 84 & 0.732 \\
First by Tideman and Chieruzzi: (D, D) & 2.596 & 94 & 0.711 & - & - & - & - \\
Adaptive Pavlov 2006 & 2.596 & 95 & 0.724 & - & - & 90 & 0.717 \\
Meta Majority Memory One: 36 players & 2.595 & 96 & 0.770 & - & - & - & - \\
Once Bitten & 2.592 & 97 & 0.790 & - & - & 67 & 0.784 \\
First by Davis: 10 & 2.591 & 98 & 0.585 & - & - & - & - \\
k53r & 2.591 & 99 & 0.705 & 45 & 0.728 & - & - \\
Soft Go By Majority: 5 & 2.590 & 100 & 0.791 & - & - & 97 & 0.783 \\
k73r & 2.588 & 101 & 0.725 & 41 & 0.764 & - & - \\
Limited Retaliate 3: 0.05, 20 & 2.584 & 102 & 0.620 & - & - & 58 & 0.624 \\
Inverse Punisher & 2.583 & 103 & 0.631 & - & - & 64 & 0.629 \\
k70r & 2.582 & 104 & 0.685 & 32 & 0.769 & - & - \\
Forgiver & 2.582 & 105 & 0.636 & - & - & 61 & 0.628 \\
k83r & 2.582 & 106 & 0.860 & 15 & 0.935 & - & - \\
Limited Retaliate 2: 0.08, 15 & 2.580 & 107 & 0.630 & - & - & 60 & 0.635 \\
Slow Tit For Two Tats 2 & 2.580 & 108 & 0.821 & - & - & 103 & 0.809 \\
First by Grofman & 2.579 & 109 & 0.890 & - & - & - & - \\
k75r & 2.579 & 110 & 0.708 & 8 & 0.802 & - & - \\
Stalker: (D,) & 2.578 & 111 & 0.843 & - & - & 99 & 0.834 \\
VeryBad & 2.575 & 112 & 0.824 & - & - & 91 & 0.827 \\
k37r & 2.574 & 113 & 0.685 & 37 & 0.791 & - & - \\
Hard Tit For 2 Tats & 2.573 & 114 & 0.843 & - & - & 108 & 0.830 \\
k57r & 2.573 & 115 & 0.761 & 31 & 0.811 & - & - \\
Soft Go By Majority: 10 & 2.572 & 116 & 0.829 & - & - & 93 & 0.824 \\
Soft Go By Majority: 20 & 2.571 & 117 & 0.825 & - & - & 98 & 0.823 \\
Soft Go By Majority: 40 & 2.571 & 118 & 0.828 & - & - & 102 & 0.824 \\
Limited Retaliate: 0.1, 20 & 2.570 & 119 & 0.629 & - & - & 66 & 0.635 \\
Nice Average Copier & 2.570 & 120 & 0.786 & - & - & 109 & 0.776 \\
Worse and Worse 3 & 2.570 & 121 & 0.786 & - & - & 107 & 0.776 \\
Punisher & 2.565 & 122 & 0.659 & - & - & 101 & 0.652 \\
Retaliate 2: 0.08 & 2.564 & 123 & 0.620 & - & - & 63 & 0.627 \\
Second by Appold & 2.564 & 124 & 0.787 & - & - & - & - \\
Retaliate 3: 0.05 & 2.564 & 125 & 0.601 & - & - & 75 & 0.603 \\
k88r & 2.564 & 126 & 0.787 & 22 & 0.861 & - & - \\
k31r & 2.563 & 127 & 0.825 & 23 & 0.920 & - & - \\
Math Constant Hunter & 2.561 & 128 & 0.761 & - & - & 85 & 0.746 \\
Forgetful Grudger & 2.560 & 129 & 0.629 & - & - & 77 & 0.636 \\
k39r & 2.558 & 130 & 0.592 & 25 & 0.676 & - & - \\
Retaliate: 0.1 & 2.557 & 131 & 0.618 & - & - & 76 & 0.625 \\
k90r & 2.555 & 132 & 0.867 & 24 & 0.964 & - & - \\
Grumpy: Nice, 10, -10 & 2.553 & 133 & 0.864 & - & - & 104 & 0.864 \\
N Tit(s) For M Tat(s): 3, 2 & 2.550 & 134 & 0.804 & - & - & 106 & 0.798 \\
Thumper & 2.549 & 135 & 0.705 & - & - & 120 & 0.690 \\
Two Tits For Tat & 2.545 & 136 & 0.676 & - & - & 121 & 0.659 \\
Inverse & 2.543 & 137 & 0.688 & - & - & 118 & 0.678 \\
Delayed AON1 & 2.543 & 138 & 0.772 & - & - & 111 & 0.771 \\
Hard Tit For Tat & 2.537 & 139 & 0.647 & - & - & 112 & 0.642 \\
Tricky Level Punisher & 2.535 & 140 & 0.778 & - & - & 116 & 0.805 \\
Appeaser & 2.530 & 141 & 0.775 & - & - & 115 & 0.774 \\
Win-Stay Lose-Shift & 2.530 & 142 & 0.775 & - & - & - & - \\
AdaptorBrief & 2.500 & 143 & 0.608 & - & - & 124 & 0.582 \\
k69r & 2.482 & 144 & 0.532 & 29 & 0.702 & - & - \\
k78r & 2.476 & 145 & 0.614 & 19 & 0.755 & - & - \\
k67r & 2.473 & 146 & 0.665 & 27 & 0.749 & - & - \\
Eventual Cycle Hunter & 2.462 & 147 & 0.915 & - & - & 123 & 0.897 \\
k82r & 2.455 & 148 & 0.445 & 49 & 0.544 & - & - \\
First by Nydegger & 2.422 & 149 & 0.959 & - & - & - & - \\
First by Graaskamp: 0.05 & 2.410 & 150 & 0.713 & - & - & - & - \\
k48r & 2.394 & 151 & 0.437 & 53 & 0.500 & - & - \\
Random Hunter & 2.388 & 152 & 0.947 & - & - & 128 & 0.947 \\
UsuallyCooperates & 2.363 & 153 & 0.959 & - & - & - & - \\
Cycle Hunter & 2.349 & 154 & 0.930 & - & - & 131 & 0.929 \\
k76r & 2.348 & 155 & 0.553 & 46 & 0.680 & - & - \\
Second by Tester & 2.348 & 156 & 0.553 & - & - & - & - \\
Defector Hunter & 2.335 & 157 & 0.990 & - & - & 132 & 0.993 \\
Raider & 2.326 & 158 & 0.406 & - & - & 130 & 0.411 \\
Alternator Hunter & 2.326 & 159 & 0.975 & - & - & 133 & 0.979 \\
AdaptorLong & 2.326 & 160 & 0.460 & - & - & 129 & 0.436 \\
Ripoff & 2.323 & 161 & 0.544 & - & - & 140 & 0.544 \\
Average Copier & 2.323 & 162 & 0.655 & - & - & 139 & 0.637 \\
k45r & 2.321 & 163 & 0.651 & 50 & 0.754 & - & - \\
k51r & 2.318 & 164 & 0.807 & 18 & 0.905 & - & - \\
Prober 2 & 2.312 & 165 & 0.711 & - & - & 138 & 0.684 \\
k33r & 2.311 & 166 & 0.363 & 59 & 0.411 & - & - \\
Knowledgeable Worse and Worse & 2.303 & 167 & 1.000 & - & - & 164 & 0.497 \\
Cooperator & 2.303 & 168 & 1.000 & - & - & 137 & 1.000 \\
k52r & 2.303 & 169 & 0.728 & 48 & 0.838 & - & - \\
k77r & 2.296 & 170 & 0.265 & 55 & 0.332 & - & - \\
Hard Prober & 2.294 & 171 & 0.400 & - & - & 134 & 0.385 \\
Sneaky Tit For Tat & 2.276 & 172 & 0.747 & - & - & 142 & 0.756 \\
k62r & 2.250 & 173 & 0.633 & 51 & 0.754 & - & - \\
DoubleResurrection & 2.246 & 174 & 0.517 & - & - & 144 & 0.499 \\
k89r & 2.217 & 175 & 0.448 & 56 & 0.498 & - & - \\
Suspicious Tit For Tat & 2.207 & 176 & 0.544 & - & - & 147 & 0.521 \\
Willing & 2.204 & 177 & 0.966 & - & - & 145 & 0.967 \\
Remorseful Prober: 0.1 & 2.197 & 178 & 0.471 & - & - & 153 & 0.446 \\
First by Feld: 1.0, 0.5, 200 & 2.196 & 179 & 0.397 & - & - & - & - \\
First by Downing & 2.174 & 180 & 0.288 & - & - & - & - \\
ZD-Mem2 & 2.168 & 181 & 0.500 & - & - & 159 & 0.481 \\
Worse and Worse 2 & 2.164 & 182 & 0.354 & - & - & 154 & 0.309 \\
Risky QLearner & 2.159 & 183 & 0.866 & - & - & 149 & 0.850 \\
Cautious QLearner & 2.159 & 184 & 0.866 & - & - & 150 & 0.850 \\
Arrogant QLearner & 2.159 & 185 & 0.866 & - & - & 151 & 0.848 \\
Hesitant QLearner & 2.159 & 186 & 0.866 & - & - & 155 & 0.849 \\
Detective & 2.157 & 187 & 0.417 & - & - & - & - \\
Random Tit for Tat: 0.5 & 2.156 & 188 & 0.520 & - & - & 156 & 0.512 \\
First by Tullock & 2.142 & 189 & 0.465 & - & - & - & - \\
k74r & 2.131 & 190 & 0.124 & 61 & 0.174 & - & - \\
k54r & 2.131 & 191 & 0.443 & 58 & 0.467 & - & - \\
Adaptive & 2.128 & 192 & 0.509 & - & - & 143 & 0.519 \\
Worse and Worse & 2.126 & 193 & 0.899 & - & - & 166 & 0.899 \\
Prober & 2.124 & 194 & 0.357 & - & - & 146 & 0.359 \\
Hard Go By Majority: 5 & 2.120 & 195 & 0.505 & - & - & 167 & 0.487 \\
Hard Go By Majority & 2.115 & 196 & 0.500 & - & - & 168 & 0.479 \\
Opposite Grudger & 2.103 & 197 & 0.931 & - & - & 169 & 0.936 \\
Stochastic Cooperator & 2.100 & 198 & 0.560 & - & - & 163 & 0.557 \\
Pun1 & 2.091 & 199 & 0.770 & - & - & 172 & 0.755 \\
Naive Prober: 0.1 & 2.089 & 200 & 0.421 & - & - & 173 & 0.396 \\
EasyGo & 2.089 & 201 & 0.917 & - & - & 162 & 0.929 \\
First by Joss: 0.9 & 2.089 & 202 & 0.421 & - & - & - & - \\
ALLCorALLD & 2.084 & 203 & 0.600 & - & - & 158 & 0.605 \\
Hard Go By Majority: 40 & 2.070 & 204 & 0.464 & - & - & 176 & 0.439 \\
Prober 4 & 2.061 & 205 & 0.218 & - & - & 148 & 0.214 \\
Prober 3 & 2.059 & 206 & 0.233 & - & - & 152 & 0.236 \\
Hard Go By Majority: 20 & 2.054 & 207 & 0.451 & - & - & 178 & 0.425 \\
Calculator & 2.052 & 208 & 0.311 & - & - & 175 & 0.293 \\
Hard Go By Majority: 10 & 2.044 & 209 & 0.436 & - & - & 182 & 0.405 \\
SolutionB5 & 2.028 & 210 & 0.400 & - & - & 185 & 0.374 \\
Winner21 & 2.019 & 211 & 0.356 & - & - & 177 & 0.343 \\
Meta Mixer: 213 players & 2.012 & 212 & 0.436 & - & - & - & - \\
Fortress3 & 1.990 & 213 & 0.322 & - & - & 171 & 0.324 \\
Fortress4 & 1.988 & 214 & 0.234 & - & - & 170 & 0.229 \\
Meta Hunter Aggressive: 7 players & 1.986 & 215 & 0.210 & - & - & 160 & 0.228 \\
Cycler CCCCCD & 1.984 & 216 & 0.836 & - & - & 191 & 0.835 \\
Stochastic WSLS: 0.05 & 1.979 & 217 & 0.560 & - & - & 181 & 0.555 \\
Cycler CCCDCD & 1.973 & 218 & 0.670 & - & - & 186 & 0.670 \\
k71r & 1.972 & 219 & 0.160 & 60 & 0.158 & - & - \\
Cycler CCCD & 1.958 & 220 & 0.752 & - & - & 193 & 0.750 \\
ZD-SET-2: 0.25, 0.0, 2 & 1.956 & 221 & 0.410 & - & - & 189 & 0.408 \\
TF2 & 1.952 & 222 & 0.189 & - & - & 184 & 0.196 \\
Cooperator Hunter & 1.946 & 223 & 0.952 & - & - & 188 & 0.962 \\
SelfSteem & 1.941 & 224 & 0.463 & - & - & 192 & 0.467 \\
SolutionB1 & 1.935 & 225 & 0.925 & - & - & 195 & 0.932 \\
Cycler CCD & 1.927 & 226 & 0.669 & - & - & 200 & 0.670 \\
Meta Winner Long Memory: 134 players & 1.926 & 227 & 0.060 & - & - & - & - \\
Meta Winner: 213 players & 1.919 & 228 & 0.059 & - & - & - & - \\
Alternator & 1.916 & 229 & 0.502 & - & - & 205 & 0.500 \\
k63r & 1.915 & 230 & 0.502 & 57 & 0.502 & - & - \\
Meta Winner Deterministic: 146 players & 1.905 & 231 & 0.052 & - & - & - & - \\
ZD-Extort-2 v2: 0.125, 0.5, 1 & 1.902 & 232 & 0.263 & - & - & 207 & 0.256 \\
ZD-Extort-2: 0.1111111111111111, 0.5 & 1.901 & 233 & 0.265 & - & - & 206 & 0.261 \\
Meta Winner Ensemble: 213 players & 1.896 & 234 & 0.032 & - & - & - & - \\
Meta Winner Stochastic: 67 players & 1.896 & 235 & 0.043 & - & - & - & - \\
Win-Shift Lose-Stay: D & 1.890 & 236 & 0.544 & - & - & 229 & 0.572 \\
Meta Winner Finite Memory: 79 players & 1.889 & 237 & 0.039 & - & - & - & - \\
Cycler DC & 1.889 & 238 & 0.498 & - & - & 211 & 0.500 \\
Meta Winner Memory One: 36 players & 1.877 & 239 & 0.022 & - & - & - & - \\
k50r & 1.876 & 240 & 0.941 & 54 & 0.930 & - & - \\
TF1 & 1.868 & 241 & 0.101 & - & - & 209 & 0.097 \\
ThueMorse & 1.868 & 242 & 0.501 & - & - & 213 & 0.500 \\
Cycler DDC & 1.855 & 243 & 0.331 & - & - & 227 & 0.330 \\
ZD-Extort3: 0.11538461538461539, 0.3333333333333333, 1 & 1.855 & 244 & 0.199 & - & - & 219 & 0.196 \\
AntiCycler & 1.852 & 245 & 0.890 & - & - & 221 & 0.900 \\
Predator & 1.851 & 246 & 0.091 & - & - & 208 & 0.085 \\
k36r & 1.849 & 247 & 0.092 & 63 & 0.092 & - & - \\
ZD-Extort-4: 0.23529411764705882, 0.25, 1 & 1.846 & 248 & 0.158 & - & - & 225 & 0.158 \\
ThueMorseInverse & 1.843 & 249 & 0.499 & - & - & 203 & 0.500 \\
CollectiveStrategy & 1.841 & 250 & 0.018 & - & - & 202 & 0.010 \\
$\pi$ & 1.840 & 251 & 0.816 & - & - & 222 & 0.817 \\
UsuallyDefects & 1.838 & 252 & 0.071 & - & - & - & - \\
Tricky Cooperator & 1.830 & 253 & 0.840 & - & - & 216 & 0.838 \\
ZD-Mischief: 0.1, 0.0, 1 & 1.825 & 254 & 0.097 & - & - & 217 & 0.096 \\
Aggravater & 1.822 & 255 & 0.089 & - & - & 212 & 0.084 \\
Better and Better & 1.819 & 256 & 0.101 & - & - & 204 & 0.100 \\
ZD-Extortion: 0.2, 0.1, 1 & 1.818 & 257 & 0.112 & - & - & 224 & 0.115 \\
$e$ & 1.817 & 258 & 0.800 & - & - & 226 & 0.799 \\
First by Anonymous & 1.817 & 259 & 0.500 & - & - & - & - \\
krandomc & 1.817 & 260 & 0.500 & 62 & 0.500 & - & - \\
Bush Mosteller: 0.5, 0.5, 3.0, 0.5 & 1.800 & 261 & 0.298 & - & - & 228 & 0.296 \\
Desperate & 1.797 & 262 & 0.375 & - & - & 220 & 0.365 \\
Gradual Killer: (D, D, D, D, D, C, C) & 1.794 & 263 & 0.563 & - & - & 223 & 0.550 \\
Meta Minority: 213 players & 1.792 & 264 & 0.664 & - & - & - & - \\
Hopeless & 1.776 & 265 & 0.753 & - & - & 233 & 0.752 \\
Bully & 1.756 & 266 & 0.620 & - & - & 218 & 0.597 \\
Defector & 1.756 & 267 & 0.000 & - & - & 232 & 0.000 \\
Handshake & 1.750 & 268 & 0.076 & - & - & 236 & 0.097 \\
Tricky Defector & 1.736 & 269 & 0.441 & - & - & 231 & 0.422 \\
$\phi$ & 1.728 & 270 & 0.728 & - & - & 234 & 0.716 \\
Negation & 1.726 & 271 & 0.628 & - & - & 230 & 0.606 \\
Anti Tit For Tat & 1.696 & 272 & 0.636 & - & - & 235 & 0.615 \\
\bottomrule
\end{tabular}


==> assets/axelord_python_tournament_rankings_full_rows.tex <==
EvolvedLookerUp2\_2\_2\textsuperscript{\textdagger} & 2.802 & 1 & 0.756 & - & - & 1 & 0.736 \\
Evolved HMM 5\textsuperscript{\textdagger} & 2.788 & 2 & 0.751 & - & - & 2 & 0.742 \\
Omega TFT: 3, 8 & 2.786 & 3 & 0.750 & - & - & 12 & 0.725 \\
Evolved ANN 5\textsuperscript{\textdagger} & 2.784 & 4 & 0.720 & - & - & 3 & 0.713 \\
Evolved ANN\textsuperscript{\textdagger} & 2.782 & 5 & 0.739 & - & - & 5 & 0.727 \\
Evolved FSM 16\textsuperscript{\textdagger} & 2.780 & 6 & 0.731 & - & - & 4 & 0.713 \\
Evolved FSM 16 Noise 05\textsuperscript{\textdagger} & 2.776 & 7 & 0.726 & - & - & 6 & 0.717 \\
PSO Gambler 2\_2\_2\textsuperscript{\textdagger} & 2.760 & 8 & 0.702 & - & - & 7 & 0.692 \\
Original Gradual & 2.757 & 9 & 0.808 & - & - & - & - \\
PSO Gambler 2\_2\_2 Noise 05\textsuperscript{\textdagger} & 2.756 & 10 & 0.740 & - & - & 14 & 0.723 \\
PSO Gambler Mem1\textsuperscript{\textdagger} & 2.756 & 11 & 0.734 & - & - & 9 & 0.728 \\
Evolved FSM 4\textsuperscript{\textdagger} & 2.752 & 12 & 0.793 & - & - & 10 & 0.777 \\
PSO Gambler 1\_1\_1\textsuperscript{\textdagger} & 2.752 & 13 & 0.704 & - & - & 8 & 0.702 \\
Gradual & 2.746 & 14 & 0.763 & - & - & 15 & 0.793 \\
DBS: 0.75, 3, 4, 3, 5 & 2.739 & 15 & 0.750 & - & - & 11 & 0.739 \\
k42r & 2.735 & 16 & 0.820 & 3 & 0.916 & - & - \\
Winner12 & 2.733 & 17 & 0.688 & - & - & 16 & 0.682 \\
Spiteful Tit For Tat & 2.723 & 18 & 0.691 & - & - & 19 & 0.664 \\
k60r & 2.723 & 19 & 0.691 & 6 & 0.844 & - & - \\
k85r & 2.716 & 20 & 0.627 & 33 & 0.726 & - & - \\
EugineNier: (D,) & 2.713 & 21 & 0.673 & - & - & 22 & 0.645 \\
k80r & 2.706 & 22 & 0.723 & 36 & 0.809 & - & - \\
k32r & 2.704 & 23 & 0.758 & 10 & 0.873 & - & - \\
DoubleCrosser: (D, D) & 2.703 & 24 & 0.693 & - & - & 13 & 0.677 \\
k58r & 2.703 & 25 & 0.746 & 21 & 0.852 & - & - \\
k87r & 2.702 & 26 & 0.691 & 44 & 0.767 & - & - \\
k40r & 2.698 & 27 & 0.665 & 35 & 0.746 & - & - \\
k65r & 2.698 & 28 & 0.645 & 47 & 0.715 & - & - \\
Forgetful Fool Me Once: 0.05 & 2.696 & 29 & 0.750 & - & - & 20 & 0.753 \\
k49r & 2.689 & 30 & 0.813 & 4 & 0.892 & - & - \\
k56r & 2.689 & 31 & 0.793 & 38 & 0.891 & - & - \\
k59r & 2.688 & 32 & 0.793 & 40 & 0.892 & - & - \\
Revised Downing & 2.688 & 33 & 0.793 & - & - & - & - \\
Fool Me Once & 2.682 & 34 & 0.627 & - & - & 17 & 0.624 \\
k41r & 2.682 & 35 & 0.768 & 7 & 0.865 & - & - \\
k55r & 2.681 & 36 & 0.817 & 42 & 0.903 & - & - \\
First by Shubik & 2.680 & 37 & 0.740 & - & - & - & - \\
ZD-GTFT-2: 0.25, 0.5 & 2.680 & 38 & 0.867 & - & - & 50 & 0.855 \\
Soft Joss: 0.9 & 2.679 & 39 & 0.844 & - & - & 53 & 0.829 \\
BackStabber: (D, D) & 2.675 & 40 & 0.654 & - & - & 18 & 0.641 \\
MEM2 & 2.671 & 41 & 0.609 & - & - & 23 & 0.597 \\
AON2 & 2.670 & 42 & 0.684 & - & - & 21 & 0.676 \\
k81r & 2.669 & 43 & 0.704 & 43 & 0.779 & - & - \\
Meta Hunter: 6 players & 2.663 & 44 & 0.647 & - & - & 29 & 0.638 \\
NMWE Finite Memory: 79 players & 2.661 & 45 & 0.587 & - & - & - & - \\
k44r & 2.660 & 46 & 0.790 & 5 & 0.882 & - & - \\
k84r & 2.659 & 47 & 0.785 & 9 & 0.882 & - & - \\
GTFT: 0.33 & 2.658 & 48 & 0.894 & - & - & 59 & 0.886 \\
EvolvedLookerUp1\_1\_1\textsuperscript{\textdagger} & 2.658 & 49 & 0.620 & - & - & 37 & 0.615 \\
NMWE Stochastic: 67 players & 2.658 & 50 & 0.590 & - & - & - & - \\
k38r & 2.656 & 51 & 0.780 & 34 & 0.874 & - & - \\
Michaelos: (D,) & 2.655 & 52 & 0.617 & - & - & 34 & 0.601 \\
First by Stein and Rapoport: 0.05: (D, D) & 2.653 & 53 & 0.766 & - & - & - & - \\
NMWE Memory One: 36 players & 2.651 & 54 & 0.579 & - & - & - & - \\
Resurrection & 2.648 & 55 & 0.771 & - & - & 71 & 0.749 \\
Nice Meta Winner Ensemble: 213 players & 2.646 & 56 & 0.578 & - & - & - & - \\
k92r & 2.645 & 57 & 0.794 & 1 & 0.922 & - & - \\
Adaptive Tit For Tat: 0.5 & 2.645 & 58 & 0.794 & - & - & 79 & 0.773 \\
Forgiving Tit For Tat & 2.643 & 59 & 0.801 & - & - & 81 & 0.778 \\
NMWE Deterministic: 146 players & 2.638 & 60 & 0.575 & - & - & - & - \\
General Soft Grudger: n=1,d=4,c=2 & 2.638 & 61 & 0.817 & - & - & 57 & 0.811 \\
Soft Grudger & 2.637 & 62 & 0.817 & - & - & 56 & 0.811 \\
Meta Majority Long Memory: 134 players & 2.637 & 63 & 0.739 & - & - & - & - \\
Firm But Fair & 2.636 & 64 & 0.867 & - & - & 86 & 0.856 \\
Level Punisher & 2.636 & 65 & 0.734 & - & - & 44 & 0.731 \\
k68r & 2.634 & 66 & 0.859 & 12 & 0.917 & - & - \\
k86r & 2.632 & 67 & 0.745 & 28 & 0.811 & - & - \\
NMWE Long Memory: 134 players & 2.632 & 68 & 0.575 & - & - & - & - \\
Meta Majority: 213 players & 2.631 & 69 & 0.757 & - & - & - & - \\
ZD-GEN-2: 0.125, 0.5, 3 & 2.630 & 70 & 0.855 & - & - & 62 & 0.850 \\
k66r & 2.629 & 71 & 0.795 & 20 & 0.866 & - & - \\
Evolved ANN 5 Noise 05\textsuperscript{\textdagger} & 2.624 & 72 & 0.565 & - & - & 45 & 0.544 \\
Second by Eatherley & 2.624 & 73 & 0.884 & - & - & - & - \\
k46r & 2.624 & 74 & 0.884 & 14 & 0.948 & - & - \\
TF3 & 2.624 & 75 & 0.585 & - & - & 38 & 0.575 \\
Memory Decay: 0.1, 0.03, -2, 1, Tit For Tat, 15 & 2.623 & 76 & 0.756 & - & - & - & - \\
Nice Meta Winner: 213 players & 2.622 & 77 & 0.586 & - & - & - & - \\
k72r & 2.622 & 78 & 0.841 & 13 & 0.924 & - & - \\
k43r & 2.622 & 79 & 0.581 & 39 & 0.667 & - & - \\
Doubler & 2.621 & 80 & 0.821 & - & - & 88 & 0.805 \\
Meta Majority Finite Memory: 79 players & 2.619 & 81 & 0.778 & - & - & - & - \\
GrudgerAlternator & 2.619 & 82 & 0.783 & - & - & 72 & 0.779 \\
k34r & 2.618 & 83 & 0.568 & 52 & 0.652 & - & - \\
k47r & 2.611 & 84 & 0.579 & 16 & 0.723 & - & - \\
k61r & 2.606 & 85 & 0.886 & 2 & 0.954 & - & - \\
Second by Champion & 2.606 & 86 & 0.883 & - & - & - & - \\
k35r & 2.605 & 87 & 0.787 & 11 & 0.888 & - & - \\
k79r & 2.604 & 88 & 0.804 & 26 & 0.875 & - & - \\
k91r & 2.603 & 89 & 0.839 & 30 & 0.873 & - & - \\
ShortMem & 2.601 & 90 & 0.817 & - & - & 83 & 0.809 \\
Dynamic Two Tits For Tat & 2.599 & 91 & 0.838 & - & - & 95 & 0.827 \\
k64r & 2.599 & 92 & 0.796 & 17 & 0.884 & - & - \\
Adaptive Pavlov 2011 & 2.597 & 93 & 0.745 & - & - & 84 & 0.732 \\
First by Tideman and Chieruzzi: (D, D) & 2.596 & 94 & 0.711 & - & - & - & - \\
Adaptive Pavlov 2006 & 2.596 & 95 & 0.724 & - & - & 90 & 0.717 \\
Meta Majority Memory One: 36 players & 2.595 & 96 & 0.770 & - & - & - & - \\
Once Bitten & 2.592 & 97 & 0.790 & - & - & 67 & 0.784 \\
First by Davis: 10 & 2.591 & 98 & 0.585 & - & - & - & - \\
k53r & 2.591 & 99 & 0.705 & 45 & 0.728 & - & - \\
Soft Go By Majority: 5 & 2.590 & 100 & 0.791 & - & - & 97 & 0.783 \\
k73r & 2.588 & 101 & 0.725 & 41 & 0.764 & - & - \\
Limited Retaliate 3: 0.05, 20 & 2.584 & 102 & 0.620 & - & - & 58 & 0.624 \\
Inverse Punisher & 2.583 & 103 & 0.631 & - & - & 64 & 0.629 \\
k70r & 2.582 & 104 & 0.685 & 32 & 0.769 & - & - \\
Forgiver & 2.582 & 105 & 0.636 & - & - & 61 & 0.628 \\
k83r & 2.582 & 106 & 0.860 & 15 & 0.935 & - & - \\
Limited Retaliate 2: 0.08, 15 & 2.580 & 107 & 0.630 & - & - & 60 & 0.635 \\
Slow Tit For Two Tats 2 & 2.580 & 108 & 0.821 & - & - & 103 & 0.809 \\
First by Grofman & 2.579 & 109 & 0.890 & - & - & - & - \\
k75r & 2.579 & 110 & 0.708 & 8 & 0.802 & - & - \\
Stalker: (D,) & 2.578 & 111 & 0.843 & - & - & 99 & 0.834 \\
VeryBad & 2.575 & 112 & 0.824 & - & - & 91 & 0.827 \\
k37r & 2.574 & 113 & 0.685 & 37 & 0.791 & - & - \\
Hard Tit For 2 Tats & 2.573 & 114 & 0.843 & - & - & 108 & 0.830 \\
k57r & 2.573 & 115 & 0.761 & 31 & 0.811 & - & - \\
Soft Go By Majority: 10 & 2.572 & 116 & 0.829 & - & - & 93 & 0.824 \\
Soft Go By Majority: 20 & 2.571 & 117 & 0.825 & - & - & 98 & 0.823 \\
Soft Go By Majority: 40 & 2.571 & 118 & 0.828 & - & - & 102 & 0.824 \\
Limited Retaliate: 0.1, 20 & 2.570 & 119 & 0.629 & - & - & 66 & 0.635 \\
Nice Average Copier & 2.570 & 120 & 0.786 & - & - & 109 & 0.776 \\
Worse and Worse 3 & 2.570 & 121 & 0.786 & - & - & 107 & 0.776 \\
Punisher & 2.565 & 122 & 0.659 & - & - & 101 & 0.652 \\
Retaliate 2: 0.08 & 2.564 & 123 & 0.620 & - & - & 63 & 0.627 \\
Second by Appold & 2.564 & 124 & 0.787 & - & - & - & - \\
Retaliate 3: 0.05 & 2.564 & 125 & 0.601 & - & - & 75 & 0.603 \\
k88r & 2.564 & 126 & 0.787 & 22 & 0.861 & - & - \\
k31r & 2.563 & 127 & 0.825 & 23 & 0.920 & - & - \\
Math Constant Hunter & 2.561 & 128 & 0.761 & - & - & 85 & 0.746 \\
Forgetful Grudger & 2.560 & 129 & 0.629 & - & - & 77 & 0.636 \\
k39r & 2.558 & 130 & 0.592 & 25 & 0.676 & - & - \\
Retaliate: 0.1 & 2.557 & 131 & 0.618 & - & - & 76 & 0.625 \\
k90r & 2.555 & 132 & 0.867 & 24 & 0.964 & - & - \\
Grumpy: Nice, 10, -10 & 2.553 & 133 & 0.864 & - & - & 104 & 0.864 \\
N Tit(s) For M Tat(s): 3, 2 & 2.550 & 134 & 0.804 & - & - & 106 & 0.798 \\
Thumper & 2.549 & 135 & 0.705 & - & - & 120 & 0.690 \\
Two Tits For Tat & 2.545 & 136 & 0.676 & - & - & 121 & 0.659 \\
Inverse & 2.543 & 137 & 0.688 & - & - & 118 & 0.678 \\
Delayed AON1 & 2.543 & 138 & 0.772 & - & - & 111 & 0.771 \\
Hard Tit For Tat & 2.537 & 139 & 0.647 & - & - & 112 & 0.642 \\
Tricky Level Punisher & 2.535 & 140 & 0.778 & - & - & 116 & 0.805 \\
Appeaser & 2.530 & 141 & 0.775 & - & - & 115 & 0.774 \\
Win-Stay Lose-Shift & 2.530 & 142 & 0.775 & - & - & - & - \\
AdaptorBrief & 2.500 & 143 & 0.608 & - & - & 124 & 0.582 \\
k69r & 2.482 & 144 & 0.532 & 29 & 0.702 & - & - \\
k78r & 2.476 & 145 & 0.614 & 19 & 0.755 & - & - \\
k67r & 2.473 & 146 & 0.665 & 27 & 0.749 & - & - \\
Eventual Cycle Hunter & 2.462 & 147 & 0.915 & - & - & 123 & 0.897 \\
k82r & 2.455 & 148 & 0.445 & 49 & 0.544 & - & - \\
First by Nydegger & 2.422 & 149 & 0.959 & - & - & - & - \\
First by Graaskamp: 0.05 & 2.410 & 150 & 0.713 & - & - & - & - \\
k48r & 2.394 & 151 & 0.437 & 53 & 0.500 & - & - \\
Random Hunter & 2.388 & 152 & 0.947 & - & - & 128 & 0.947 \\
UsuallyCooperates & 2.363 & 153 & 0.959 & - & - & - & - \\
Cycle Hunter & 2.349 & 154 & 0.930 & - & - & 131 & 0.929 \\
k76r & 2.348 & 155 & 0.553 & 46 & 0.680 & - & - \\
Second by Tester & 2.348 & 156 & 0.553 & - & - & - & - \\
Defector Hunter & 2.335 & 157 & 0.990 & - & - & 132 & 0.993 \\
Raider & 2.326 & 158 & 0.406 & - & - & 130 & 0.411 \\
Alternator Hunter & 2.326 & 159 & 0.975 & - & - & 133 & 0.979 \\
AdaptorLong & 2.326 & 160 & 0.460 & - & - & 129 & 0.436 \\
Ripoff & 2.323 & 161 & 0.544 & - & - & 140 & 0.544 \\
Average Copier & 2.323 & 162 & 0.655 & - & - & 139 & 0.637 \\
k45r & 2.321 & 163 & 0.651 & 50 & 0.754 & - & - \\
k51r & 2.318 & 164 & 0.807 & 18 & 0.905 & - & - \\
Prober 2 & 2.312 & 165 & 0.711 & - & - & 138 & 0.684 \\
k33r & 2.311 & 166 & 0.363 & 59 & 0.411 & - & - \\
Knowledgeable Worse and Worse & 2.303 & 167 & 1.000 & - & - & 164 & 0.497 \\
Cooperator & 2.303 & 168 & 1.000 & - & - & 137 & 1.000 \\
k52r & 2.303 & 169 & 0.728 & 48 & 0.838 & - & - \\
k77r & 2.296 & 170 & 0.265 & 55 & 0.332 & - & - \\
Hard Prober & 2.294 & 171 & 0.400 & - & - & 134 & 0.385 \\
Sneaky Tit For Tat & 2.276 & 172 & 0.747 & - & - & 142 & 0.756 \\
k62r & 2.250 & 173 & 0.633 & 51 & 0.754 & - & - \\
DoubleResurrection & 2.246 & 174 & 0.517 & - & - & 144 & 0.499 \\
k89r & 2.217 & 175 & 0.448 & 56 & 0.498 & - & - \\
Suspicious Tit For Tat & 2.207 & 176 & 0.544 & - & - & 147 & 0.521 \\
Willing & 2.204 & 177 & 0.966 & - & - & 145 & 0.967 \\
Remorseful Prober: 0.1 & 2.197 & 178 & 0.471 & - & - & 153 & 0.446 \\
First by Feld: 1.0, 0.5, 200 & 2.196 & 179 & 0.397 & - & - & - & - \\
First by Downing & 2.174 & 180 & 0.288 & - & - & - & - \\
ZD-Mem2 & 2.168 & 181 & 0.500 & - & - & 159 & 0.481 \\
Worse and Worse 2 & 2.164 & 182 & 0.354 & - & - & 154 & 0.309 \\
Risky QLearner & 2.159 & 183 & 0.866 & - & - & 149 & 0.850 \\
Cautious QLearner & 2.159 & 184 & 0.866 & - & - & 150 & 0.850 \\
Arrogant QLearner & 2.159 & 185 & 0.866 & - & - & 151 & 0.848 \\
Hesitant QLearner & 2.159 & 186 & 0.866 & - & - & 155 & 0.849 \\
Detective & 2.157 & 187 & 0.417 & - & - & - & - \\
Random Tit for Tat: 0.5 & 2.156 & 188 & 0.520 & - & - & 156 & 0.512 \\
First by Tullock & 2.142 & 189 & 0.465 & - & - & - & - \\
k74r & 2.131 & 190 & 0.124 & 61 & 0.174 & - & - \\
k54r & 2.131 & 191 & 0.443 & 58 & 0.467 & - & - \\
Adaptive & 2.128 & 192 & 0.509 & - & - & 143 & 0.519 \\
Worse and Worse & 2.126 & 193 & 0.899 & - & - & 166 & 0.899 \\
Prober & 2.124 & 194 & 0.357 & - & - & 146 & 0.359 \\
Hard Go By Majority: 5 & 2.120 & 195 & 0.505 & - & - & 167 & 0.487 \\
Hard Go By Majority & 2.115 & 196 & 0.500 & - & - & 168 & 0.479 \\
Opposite Grudger & 2.103 & 197 & 0.931 & - & - & 169 & 0.936 \\
Stochastic Cooperator & 2.100 & 198 & 0.560 & - & - & 163 & 0.557 \\
Pun1 & 2.091 & 199 & 0.770 & - & - & 172 & 0.755 \\
Naive Prober: 0.1 & 2.089 & 200 & 0.421 & - & - & 173 & 0.396 \\
EasyGo & 2.089 & 201 & 0.917 & - & - & 162 & 0.929 \\
First by Joss: 0.9 & 2.089 & 202 & 0.421 & - & - & - & - \\
ALLCorALLD & 2.084 & 203 & 0.600 & - & - & 158 & 0.605 \\
Hard Go By Majority: 40 & 2.070 & 204 & 0.464 & - & - & 176 & 0.439 \\
Prober 4 & 2.061 & 205 & 0.218 & - & - & 148 & 0.214 \\
Prober 3 & 2.059 & 206 & 0.233 & - & - & 152 & 0.236 \\
Hard Go By Majority: 20 & 2.054 & 207 & 0.451 & - & - & 178 & 0.425 \\
Calculator & 2.052 & 208 & 0.311 & - & - & 175 & 0.293 \\
Hard Go By Majority: 10 & 2.044 & 209 & 0.436 & - & - & 182 & 0.405 \\
SolutionB5 & 2.028 & 210 & 0.400 & - & - & 185 & 0.374 \\
Winner21 & 2.019 & 211 & 0.356 & - & - & 177 & 0.343 \\
Meta Mixer: 213 players & 2.012 & 212 & 0.436 & - & - & - & - \\
Fortress3 & 1.990 & 213 & 0.322 & - & - & 171 & 0.324 \\
Fortress4 & 1.988 & 214 & 0.234 & - & - & 170 & 0.229 \\
Meta Hunter Aggressive: 7 players & 1.986 & 215 & 0.210 & - & - & 160 & 0.228 \\
Cycler CCCCCD & 1.984 & 216 & 0.836 & - & - & 191 & 0.835 \\
Stochastic WSLS: 0.05 & 1.979 & 217 & 0.560 & - & - & 181 & 0.555 \\
Cycler CCCDCD & 1.973 & 218 & 0.670 & - & - & 186 & 0.670 \\
k71r & 1.972 & 219 & 0.160 & 60 & 0.158 & - & - \\
Cycler CCCD & 1.958 & 220 & 0.752 & - & - & 193 & 0.750 \\
ZD-SET-2: 0.25, 0.0, 2 & 1.956 & 221 & 0.410 & - & - & 189 & 0.408 \\
TF2 & 1.952 & 222 & 0.189 & - & - & 184 & 0.196 \\
Cooperator Hunter & 1.946 & 223 & 0.952 & - & - & 188 & 0.962 \\
SelfSteem & 1.941 & 224 & 0.463 & - & - & 192 & 0.467 \\
SolutionB1 & 1.935 & 225 & 0.925 & - & - & 195 & 0.932 \\
Cycler CCD & 1.927 & 226 & 0.669 & - & - & 200 & 0.670 \\
Meta Winner Long Memory: 134 players & 1.926 & 227 & 0.060 & - & - & - & - \\
Meta Winner: 213 players & 1.919 & 228 & 0.059 & - & - & - & - \\
Alternator & 1.916 & 229 & 0.502 & - & - & 205 & 0.500 \\
k63r & 1.915 & 230 & 0.502 & 57 & 0.502 & - & - \\
Meta Winner Deterministic: 146 players & 1.905 & 231 & 0.052 & - & - & - & - \\
ZD-Extort-2 v2: 0.125, 0.5, 1 & 1.902 & 232 & 0.263 & - & - & 207 & 0.256 \\
ZD-Extort-2: 0.1111111111111111, 0.5 & 1.901 & 233 & 0.265 & - & - & 206 & 0.261 \\
Meta Winner Ensemble: 213 players & 1.896 & 234 & 0.032 & - & - & - & - \\
Meta Winner Stochastic: 67 players & 1.896 & 235 & 0.043 & - & - & - & - \\
Win-Shift Lose-Stay: D & 1.890 & 236 & 0.544 & - & - & 229 & 0.572 \\
Meta Winner Finite Memory: 79 players & 1.889 & 237 & 0.039 & - & - & - & - \\
Cycler DC & 1.889 & 238 & 0.498 & - & - & 211 & 0.500 \\
Meta Winner Memory One: 36 players & 1.877 & 239 & 0.022 & - & - & - & - \\
k50r & 1.876 & 240 & 0.941 & 54 & 0.930 & - & - \\
TF1 & 1.868 & 241 & 0.101 & - & - & 209 & 0.097 \\
ThueMorse & 1.868 & 242 & 0.501 & - & - & 213 & 0.500 \\
Cycler DDC & 1.855 & 243 & 0.331 & - & - & 227 & 0.330 \\
ZD-Extort3: 0.11538461538461539, 0.3333333333333333, 1 & 1.855 & 244 & 0.199 & - & - & 219 & 0.196 \\
AntiCycler & 1.852 & 245 & 0.890 & - & - & 221 & 0.900 \\
Predator & 1.851 & 246 & 0.091 & - & - & 208 & 0.085 \\
k36r & 1.849 & 247 & 0.092 & 63 & 0.092 & - & - \\
ZD-Extort-4: 0.23529411764705882, 0.25, 1 & 1.846 & 248 & 0.158 & - & - & 225 & 0.158 \\
ThueMorseInverse & 1.843 & 249 & 0.499 & - & - & 203 & 0.500 \\
CollectiveStrategy & 1.841 & 250 & 0.018 & - & - & 202 & 0.010 \\
$\pi$ & 1.840 & 251 & 0.816 & - & - & 222 & 0.817 \\
UsuallyDefects & 1.838 & 252 & 0.071 & - & - & - & - \\
Tricky Cooperator & 1.830 & 253 & 0.840 & - & - & 216 & 0.838 \\
ZD-Mischief: 0.1, 0.0, 1 & 1.825 & 254 & 0.097 & - & - & 217 & 0.096 \\
Aggravater & 1.822 & 255 & 0.089 & - & - & 212 & 0.084 \\
Better and Better & 1.819 & 256 & 0.101 & - & - & 204 & 0.100 \\
ZD-Extortion: 0.2, 0.1, 1 & 1.818 & 257 & 0.112 & - & - & 224 & 0.115 \\
$e$ & 1.817 & 258 & 0.800 & - & - & 226 & 0.799 \\
First by Anonymous & 1.817 & 259 & 0.500 & - & - & - & - \\
krandomc & 1.817 & 260 & 0.500 & 62 & 0.500 & - & - \\
Bush Mosteller: 0.5, 0.5, 3.0, 0.5 & 1.800 & 261 & 0.298 & - & - & 228 & 0.296 \\
Desperate & 1.797 & 262 & 0.375 & - & - & 220 & 0.365 \\
Gradual Killer: (D, D, D, D, D, C, C) & 1.794 & 263 & 0.563 & - & - & 223 & 0.550 \\
Meta Minority: 213 players & 1.792 & 264 & 0.664 & - & - & - & - \\
Hopeless & 1.776 & 265 & 0.753 & - & - & 233 & 0.752 \\
Bully & 1.756 & 266 & 0.620 & - & - & 218 & 0.597 \\
Defector & 1.756 & 267 & 0.000 & - & - & 232 & 0.000 \\
Handshake & 1.750 & 268 & 0.076 & - & - & 236 & 0.097 \\
Tricky Defector & 1.736 & 269 & 0.441 & - & - & 231 & 0.422 \\
$\phi$ & 1.728 & 270 & 0.728 & - & - & 234 & 0.716 \\
Negation & 1.726 & 271 & 0.628 & - & - & 230 & 0.606 \\
Anti Tit For Tat & 1.696 & 272 & 0.636 & - & - & 235 & 0.615 \\

==> assets/extra_strategies_summary_full_table.tex <==
\begin{tabular}{lrrrrr}
\toprule
 & 0 New (N = 1) & 1 New (N = 209) & 2 New (N = 21736) & 3 New (N = 1499784) & 4 New (N = 77238876) \\
\midrule
k32r & 0.008 & 0.000 & 0.000 & 0.000 & 0.001 \\
k41r & 0.000 & 0.000 & 0.000 & 0.000 & 0.000 \\
k42r & 0.315 & 0.148 & 0.269 & 0.366 & 0.217 \\
k44r & 0.004 & 0.000 & 0.000 & 0.001 & 0.005 \\
k49r & 0.000 & 0.000 & 0.000 & 0.000 & 0.000 \\
k60r & 0.010 & 0.005 & 0.011 & 0.019 & 0.005 \\
k75r & 0.023 & 0.000 & 0.001 & 0.002 & 0.001 \\
k92r & 0.633 & 0.847 & 0.717 & 0.608 & 0.754 \\
Sum & 0.993 & 1.000 & 0.999 & 0.997 & 0.982 \\
\bottomrule
\end{tabular}


==> assets/full_tournament_rankings.tex <==
\begin{tabular}{lrrrrrrr}
\toprule
 & Mean Score & Rank & Coop. Rate & Original Rank & Reproduced Coop. Rate & Library Rank & Library Coop. Rate \\
\midrule
EvolvedLookerUp2\_2\_2\textsuperscript{\textdagger} & 2.802 & 1 & 0.756 & NA & NA & 1 & 0.736 \\
Evolved HMM 5\textsuperscript{\textdagger} & 2.788 & 2 & 0.751 & NA & NA & 2 & 0.742 \\
Omega TFT: 3, 8 & 2.786 & 3 & 0.750 & NA & NA & 12 & 0.725 \\
Evolved ANN 5\textsuperscript{\textdagger} & 2.784 & 4 & 0.720 & NA & NA & 3 & 0.713 \\
Evolved ANN\textsuperscript{\textdagger} & 2.782 & 5 & 0.739 & NA & NA & 5 & 0.727 \\
Evolved FSM 16\textsuperscript{\textdagger} & 2.780 & 6 & 0.731 & NA & NA & 4 & 0.713 \\
Evolved FSM 16 Noise 05\textsuperscript{\textdagger} & 2.776 & 7 & 0.726 & NA & NA & 6 & 0.717 \\
PSO Gambler 2\_2\_2\textsuperscript{\textdagger} & 2.760 & 8 & 0.702 & NA & NA & 7 & 0.692 \\
Original Gradual & 2.757 & 9 & 0.808 & NA & NA & NA & NA \\
PSO Gambler 2\_2\_2 Noise 05\textsuperscript{\textdagger} & 2.756 & 10 & 0.740 & NA & NA & 14 & 0.723 \\
PSO Gambler Mem1\textsuperscript{\textdagger} & 2.756 & 11 & 0.734 & NA & NA & 9 & 0.728 \\
Evolved FSM 4\textsuperscript{\textdagger} & 2.752 & 12 & 0.793 & NA & NA & 10 & 0.777 \\
PSO Gambler 1\_1\_1\textsuperscript{\textdagger} & 2.752 & 13 & 0.704 & NA & NA & 8 & 0.702 \\
Gradual & 2.746 & 14 & 0.763 & NA & NA & 15 & 0.793 \\
DBS: 0.75, 3, 4, 3, 5 & 2.739 & 15 & 0.750 & NA & NA & 11 & 0.739 \\
k42r & 2.735 & 16 & 0.820 & 3 & 0.916 & NA & NA \\
Winner12 & 2.733 & 17 & 0.688 & NA & NA & 16 & 0.682 \\
Spiteful Tit For Tat & 2.723 & 18 & 0.691 & NA & NA & 19 & 0.664 \\
k60r & 2.723 & 19 & 0.691 & 6 & 0.844 & NA & NA \\
k85r & 2.716 & 20 & 0.627 & 33 & 0.726 & NA & NA \\
EugineNier: (D,) & 2.713 & 21 & 0.673 & NA & NA & 22 & 0.645 \\
k80r & 2.706 & 22 & 0.723 & 36 & 0.809 & NA & NA \\
k32r & 2.704 & 23 & 0.758 & 10 & 0.873 & NA & NA \\
DoubleCrosser: (D, D) & 2.703 & 24 & 0.693 & NA & NA & 13 & 0.677 \\
k58r & 2.703 & 25 & 0.746 & 21 & 0.852 & NA & NA \\
\bottomrule
\end{tabular}


==> assets/list_of_all_players.tex <==
\item EvolvedLookerUp2\_2\_2: 1 / 30 / 118
\item Evolved HMM 5: 2 / 13 / 59
\item Omega TFT: 3, 8: 3 / 4 / 17
\item Evolved ANN 5: 4 / 7 / 36
\item Evolved ANN: 5 / 3 / 8
\item Evolved FSM 16: 6 / 15 / 78
\item Evolved FSM 16 Noise 05: 7 / 1 / 4
\item PSO Gambler 2\_2\_2: 8 / 53 / 138
\item Original Gradual: 9 / 20 / 30
\item PSO Gambler 2\_2\_2 Noise 05: 10 / 9 / 24
\item PSO Gambler Mem1: 11 / 39 / 107
\item Evolved FSM 4: 12 / 28 / 85
\item PSO Gambler 1\_1\_1: 13 / 61 / 140
\item Gradual: 14 / 17 / 29
\item DBS: 0.75, 3, 4, 3, 5: 15 / 2 / 1
\item k42r: 16 / 25 / 21 / 3
\item Winner12: 17 / 60 / 127
\item Spiteful Tit For Tat: 18 / 24 / 22
\item k60r: 19 / 31 / 25 / 6
\item k85r: 20 / 57 / 101 / 33
\item EugineNier: (D,): 21 / 35 / 27
\item k80r: 22 / 10 / 3 / 36
\item k32r: 23 / 40 / 34 / 10
\item DoubleCrosser: (D, D): 24 / 11 / 13
\item k58r: 25 / 38 / 43 / 21
\item k87r: 26 / 74 / 124 / 44
\item k40r: 27 / 34 / 80 / 35
\item k65r: 28 / 5 / 18 / 47
\item Forgetful Fool Me Once: 0.05: 29 / 19 / 41
\item k49r: 30 / 32 / 23 / 4
\item k56r: 31 / 21 / 12 / 38
\item k59r: 32 / 23 / 11 / 40
\item Revised Downing: 33 / 22 / 10
\item Fool Me Once: 34 / 14 / 37
\item k41r: 35 / 33 / 40 / 7
\item k55r: 36 / 27 / 15 / 42
\item First by Shubik: 37 / 87 / 95
\item ZD-GTFT-2: 0.25, 0.5: 38 / 48 / 63
\item Soft Joss: 0.9: 39 / 49 / 56
\item BackStabber: (D, D): 40 / 8 / 9
\item MEM2: 41 / 79 / 103
\item AON2: 42 / 116 / 168
\item k81r: 43 / 6 / 14 / 43
\item Meta Hunter: 6 players: 44 / 69 / 108
\item NMWE Finite Memory: 79 players: 45 / 91 / 126
\item k44r: 46 / 37 / 26 / 5
\item k84r: 47 / 43 / 76 / 9
\item GTFT: 0.33: 48 / 55 / 72
\item EvolvedLookerUp1\_1\_1: 49 / 115 / 147
\item NMWE Stochastic: 67 players: 50 / 97 / 123
\item k38r: 51 / 26 / 7 / 34
\item Michaelos: (D,): 52 / 86 / 97
\item First by Stein and Rapoport: 0.05: (D, D): 53 / 47 / 44
\item NMWE Memory One: 36 players: 54 / 90 / 104
\item Resurrection: 55 / 65 / 67
\item Nice Meta Winner Ensemble: 213 players: 56 / 98 / 111
\item k92r: 57 / 70 / 69 / 1
\item Adaptive Tit For Tat: 0.5: 58 / 72 / 68
\item Forgiving Tit For Tat: 59 / 46 / 58
\item NMWE Deterministic: 146 players: 60 / 93 / 109
\item General Soft Grudger: n=1,d=4,c=2: 61 / 110 / 144
\item Soft Grudger: 62 / 109 / 142
\item Meta Majority Long Memory: 134 players: 63 / 62 / 62
\item Firm But Fair: 64 / 100 / 91
\item Level Punisher: 65 / 29 / 16
\item k68r: 66 / 117 / 139 / 12
\item k86r: 67 / 36 / 49 / 28
\item NMWE Long Memory: 134 players: 68 / 105 / 112
\item Meta Majority: 213 players: 69 / 66 / 75
\item ZD-GEN-2: 0.125, 0.5, 3: 70 / 99 / 110
\item k66r: 71 / 41 / 19 / 20
\item Evolved ANN 5 Noise 05: 72 / 12 / 2
\item Second by Eatherley: 73 / 64 / 79
\item k46r: 74 / 63 / 77 / 14
\item TF3: 75 / 75 / 90
\item Memory Decay: 0.1, 0.03, -2, 1, Tit For Tat, 15: 76 / 51 / 51
\item Nice Meta Winner: 213 players: 77 / 114 / 129
\item k72r: 78 / 77 / 38 / 13
\item k43r: 79 / 18 / 6 / 39
\item Doubler: 80 / 54 / 42
\item Meta Majority Finite Memory: 79 players: 81 / 59 / 64
\item GrudgerAlternator: 82 / 124 / 159
\item k34r: 83 / 111 / 119 / 52
\item k47r: 84 / 16 / 5 / 16
\item k61r: 85 / 126 / 156 / 2
\item Second by Champion: 86 / 108 / 93
\item k35r: 87 / 95 / 89 / 11
\item k79r: 88 / 52 / 54 / 26
\item k91r: 89 / 67 / 52 / 30
\item ShortMem: 90 / 56 / 32
\item Dynamic Two Tits For Tat: 91 / 94 / 92
\item k64r: 92 / 71 / 46 / 17
\item Adaptive Pavlov 2011: 93 / 112 / 121
\item First by Tideman and Chieruzzi: (D, D): 94 / 120 / 102
\item Adaptive Pavlov 2006: 95 / 113 / 131
\item Meta Majority Memory One: 36 players: 96 / 101 / 87
\item Once Bitten: 97 / 45 / 39
\item First by Davis: 10: 98 / 127 / 122
\item k53r: 99 / 128 / 128 / 45
\item Soft Go By Majority: 5: 100 / 50 / 35
\item k73r: 101 / 44 / 50 / 41
\item Limited Retaliate 3: 0.05, 20: 102 / 130 / 152
\item Inverse Punisher: 103 / 132 / 157
\item k70r: 104 / 129 / 149 / 32
\item Forgiver: 105 / 82 / 96
\item k83r: 106 / 92 / 83 / 15
\item Limited Retaliate 2: 0.08, 15: 107 / 134 / 164
\item Slow Tit For Two Tats 2: 108 / 68 / 74
\item First by Grofman: 109 / 135 / 176
\item k75r: 110 / 42 / 31 / 8
\item Stalker: (D,): 111 / 88 / 65
\item VeryBad: 112 / 89 / 60
\item k37r: 113 / 73 / 57 / 37
\item Hard Tit For 2 Tats: 114 / 83 / 70
\item k57r: 115 / 147 / 182 / 31
\item Soft Go By Majority: 10: 116 / 76 / 47
\item Soft Go By Majority: 20: 117 / 84 / 55
\item Soft Go By Majority: 40: 118 / 96 / 66
\item Limited Retaliate: 0.1, 20: 119 / 138 / 170
\item Nice Average Copier: 120 / 123 / 133
\item Worse and Worse 3: 121 / 125 / 132
\item Punisher: 122 / 137 / 167
\item Retaliate 2: 0.08: 123 / 139 / 163
\item Second by Appold: 124 / 119 / 106
\item Retaliate 3: 0.05: 125 / 133 / 153
\item k88r: 126 / 122 / 113 / 22
\item k31r: 127 / 107 / 73 / 23
\item Math Constant Hunter: 128 / 136 / 146
\item Forgetful Grudger: 129 / 144 / 172
\item k39r: 130 / 81 / 20 / 25
\item Retaliate: 0.1: 131 / 143 / 171
\item k90r: 132 / 104 / 71 / 24
\item Grumpy: Nice, 10, -10: 133 / 118 / 88
\item N Tit(s) For M Tat(s): 3, 2: 134 / 85 / 81
\item Thumper: 135 / 148 / 161
\item Two Tits For Tat: 136 / 146 / 165
\item Inverse: 137 / 140 / 148
\item Delayed AON1: 138 / 152 / 215
\item Hard Tit For Tat: 139 / 150 / 178
\item Tricky Level Punisher: 140 / 106 / 117
\item Appeaser: 141 / 155 / 205
\item Win-Stay Lose-Shift: 142 / 156 / 206
\item AdaptorBrief: 143 / 78 / 53
\item k69r: 144 / 121 / 48 / 29
\item k78r: 145 / 80 / 61 / 19
\item k67r: 146 / 103 / 33 / 27
\item Eventual Cycle Hunter: 147 / 157 / 198
\item k82r: 148 / 58 / 28 / 49
\item First by Nydegger: 149 / 153 / 173
\item First by Graaskamp: 0.05: 150 / 102 / 82
\item k48r: 151 / 141 / 94 / 53
\item Random Hunter: 152 / 154 / 154
\item UsuallyCooperates: 153 / 183 / 230
\item Cycle Hunter: 154 / 169 / 193
\item k76r: 155 / 166 / 155 / 46
\item Second by Tester: 156 / 163 / 151
\item Defector Hunter: 157 / 173 / 204
\item Raider: 158 / 161 / 134
\item Alternator Hunter: 159 / 175 / 200
\item AdaptorLong: 160 / 149 / 169
\item Ripoff: 161 / 172 / 162
\item Average Copier: 162 / 171 / 177
\item k45r: 163 / 159 / 115 / 50
\item k51r: 164 / 167 / 158 / 18
\item Prober 2: 165 / 162 / 130
\item k33r: 166 / 178 / 145 / 59
\item Knowledgeable Worse and Worse: 167 / 181 / 214
\item Cooperator: 168 / 179 / 211
\item k52r: 169 / 151 / 100 / 48
\item k77r: 170 / 131 / 45 / 55
\item Hard Prober: 171 / 164 / 125
\item Sneaky Tit For Tat: 172 / 180 / 179
\item k62r: 173 / 158 / 99 / 51
\item DoubleResurrection: 174 / 165 / 105
\item k89r: 175 / 200 / 191 / 56
\item Suspicious Tit For Tat: 176 / 185 / 160
\item Willing: 177 / 192 / 203
\item Remorseful Prober: 0.1: 178 / 168 / 114
\item First by Feld: 1.0, 0.5, 200: 179 / 145 / 84
\item First by Downing: 180 / 174 / 86
\item ZD-Mem2: 181 / 170 / 141
\item Worse and Worse 2: 182 / 142 / 98
\item Risky QLearner: 183 / 195 / 217
\item Cautious QLearner: 184 / 194 / 218
\item Arrogant QLearner: 185 / 196 / 216
\item Hesitant QLearner: 186 / 197 / 219
\item Detective: 187 / 189 / 166
\item Random Tit for Tat: 0.5: 188 / 188 / 180
\item First by Tullock: 189 / 160 / 116
\item k74r: 190 / 186 / 120 / 61
\item k54r: 191 / 191 / 143 / 58
\item Adaptive: 192 / 184 / 150
\item Worse and Worse: 193 / 190 / 212
\item Prober: 194 / 193 / 174
\item Hard Go By Majority: 5: 195 / 198 / 181
\item Hard Go By Majority: 196 / 202 / 194
\item Opposite Grudger: 197 / 208 / 236
\item Stochastic Cooperator: 198 / 187 / 187
\item Pun1: 199 / 206 / 199
\item Naive Prober: 0.1: 200 / 177 / 137
\item EasyGo: 201 / 220 / 259
\item First by Joss: 0.9: 202 / 176 / 136
\item ALLCorALLD: 203 / 211 / 228
\item Hard Go By Majority: 40: 204 / 201 / 188
\item Prober 4: 205 / 203 / 183
\item Prober 3: 206 / 199 / 175
\item Hard Go By Majority: 20: 207 / 207 / 185
\item Calculator: 208 / 182 / 135
\item Hard Go By Majority: 10: 209 / 209 / 186
\item SolutionB5: 210 / 210 / 184
\item Winner21: 211 / 221 / 225
\item Meta Mixer: 213 players: 212 / 205 / 195
\item Fortress3: 213 / 223 / 226
\item Fortress4: 214 / 224 / 222
\item Meta Hunter Aggressive: 7 players: 215 / 212 / 202
\item Cycler CCCCCD: 216 / 219 / 238
\item Stochastic WSLS: 0.05: 217 / 204 / 229
\item Cycler CCCDCD: 218 / 227 / 244
\item k71r: 219 / 222 / 220 / 60
\item Cycler CCCD: 220 / 228 / 245
\item ZD-SET-2: 0.25, 0.0, 2: 221 / 215 / 210
\item TF2: 222 / 229 / 231
\item Cooperator Hunter: 223 / 241 / 253
\item SelfSteem: 224 / 230 / 234
\item SolutionB1: 225 / 243 / 258
\item Cycler CCD: 226 / 231 / 239
\item Meta Winner Long Memory: 134 players: 227 / 216 / 189
\item Meta Winner: 213 players: 228 / 217 / 192
\item Alternator: 229 / 236 / 241
\item k63r: 230 / 240 / 248 / 57
\item Meta Winner Deterministic: 146 players: 231 / 218 / 190
\item ZD-Extort-2 v2: 0.125, 0.5, 1: 232 / 214 / 196
\item ZD-Extort-2: 0.1111111111111111, 0.5: 233 / 213 / 197
\item Meta Winner Ensemble: 213 players: 234 / 232 / 208
\item Meta Winner Stochastic: 67 players: 235 / 233 / 209
\item Win-Shift Lose-Stay: D: 236 / 244 / 247
\item Meta Winner Finite Memory: 79 players: 237 / 225 / 201
\item Cycler DC: 238 / 242 / 246
\item Meta Winner Memory One: 36 players: 239 / 234 / 207
\item k50r: 240 / 235 / 249 / 54
\item TF1: 241 / 238 / 224
\item ThueMorse: 242 / 250 / 256
\item Cycler DDC: 243 / 257 / 257
\item ZD-Extort3: 0.11538461538461539, 0.3333333333333333, 1: 244 / 226 / 213
\item AntiCycler: 245 / 259 / 263
\item Predator: 246 / 247 / 235
\item k36r: 247 / 251 / 243 / 63
\item ZD-Extort-4: 0.23529411764705882, 0.25, 1: 248 / 239 / 221
\item ThueMorseInverse: 249 / 248 / 251
\item CollectiveStrategy: 250 / 246 / 227
\item $\pi$: 251 / 260 / 264
\item UsuallyDefects: 252 / 249 / 237
\item Tricky Cooperator: 253 / 256 / 260
\item ZD-Mischief: 0.1, 0.0, 1: 254 / 237 / 223
\item Aggravater: 255 / 254 / 233
\item Better and Better: 256 / 258 / 242
\item ZD-Extortion: 0.2, 0.1, 1: 257 / 245 / 232
\item $e$: 258 / 261 / 265
\item First by Anonymous: 259 / 253 / 254
\item krandomc: 260 / 252 / 255 / 62
\item Bush Mosteller: 0.5, 0.5, 3.0, 0.5: 261 / 255 / 250
\item Desperate: 262 / 263 / 262
\item Gradual Killer: (D, D, D, D, D, C, C): 263 / 266 / 267
\item Meta Minority: 213 players: 264 / 268 / 268
\item Hopeless: 265 / 265 / 266
\item Bully: 266 / 269 / 269
\item Defector: 267 / 262 / 240
\item Handshake: 268 / 264 / 252
\item Tricky Defector: 269 / 267 / 261
\item $\phi$: 270 / 270 / 271
\item Negation: 271 / 271 / 270
\item Anti Tit For Tat: 272 / 272 / 272


==> assets/list_of_all_strategies.tex <==
\item EvolvedLookerUp2_2_2: 1 / 30 / 118
\item Evolved HMM 5: 2 / 13 / 59
\item Omega TFT: 3, 8: 3 / 4 / 17
\item Evolved ANN 5: 4 / 7 / 36
\item Evolved ANN: 5 / 3 / 8
\item Evolved FSM 16: 6 / 15 / 78
\item Evolved FSM 16 Noise 05: 7 / 1 / 4
\item PSO Gambler 2_2_2: 8 / 53 / 138
\item Original Gradual: 9 / 20 / 30
\item PSO Gambler 2_2_2 Noise 05: 10 / 9 / 24
\item PSO Gambler Mem1: 11 / 39 / 107
\item Evolved FSM 4: 12 / 28 / 85
\item PSO Gambler 1_1_1: 13 / 61 / 140
\item Gradual: 14 / 17 / 29
\item DBS: 0.75, 3, 4, 3, 5: 15 / 2 / 1
\item k42r: 16 / 25 / 21 / 3
\item Winner12: 17 / 60 / 127
\item Spiteful Tit For Tat: 18 / 24 / 22
\item k60r: 19 / 31 / 25 / 6
\item k85r: 20 / 57 / 101 / 33
\item EugineNier: (D,): 21 / 35 / 27
\item k80r: 22 / 10 / 3 / 36
\item k32r: 23 / 40 / 34 / 10
\item DoubleCrosser: (D, D): 24 / 11 / 13
\item k58r: 25 / 38 / 43 / 21
\item k87r: 26 / 74 / 124 / 44
\item k40r: 27 / 34 / 80 / 35
\item k65r: 28 / 5 / 18 / 47
\item Forgetful Fool Me Once: 0.05: 29 / 19 / 41
\item k49r: 30 / 32 / 23 / 4
\item k56r: 31 / 21 / 12 / 38
\item k59r: 32 / 23 / 11 / 40
\item Revised Downing: 33 / 22 / 10
\item Fool Me Once: 34 / 14 / 37
\item k41r: 35 / 33 / 40 / 7
\item k55r: 36 / 27 / 15 / 42
\item First by Shubik: 37 / 87 / 95
\item ZD-GTFT-2: 0.25, 0.5: 38 / 48 / 63
\item Soft Joss: 0.9: 39 / 49 / 56
\item BackStabber: (D, D): 40 / 8 / 9
\item MEM2: 41 / 79 / 103
\item AON2: 42 / 116 / 168
\item k81r: 43 / 6 / 14 / 43
\item Meta Hunter: 6 players: 44 / 69 / 108
\item NMWE Finite Memory: 79 players: 45 / 91 / 126
\item k44r: 46 / 37 / 26 / 5
\item k84r: 47 / 43 / 76 / 9
\item GTFT: 0.33: 48 / 55 / 72
\item EvolvedLookerUp1_1_1: 49 / 115 / 147
\item NMWE Stochastic: 67 players: 50 / 97 / 123
\item k38r: 51 / 26 / 7 / 34
\item Michaelos: (D,): 52 / 86 / 97
\item First by Stein and Rapoport: 0.05: (D, D): 53 / 47 / 44
\item NMWE Memory One: 36 players: 54 / 90 / 104
\item Resurrection: 55 / 65 / 67
\item Nice Meta Winner Ensemble: 213 players: 56 / 98 / 111
\item k92r: 57 / 70 / 69 / 1
\item Adaptive Tit For Tat: 0.5: 58 / 72 / 68
\item Forgiving Tit For Tat: 59 / 46 / 58
\item NMWE Deterministic: 146 players: 60 / 93 / 109
\item General Soft Grudger: n=1,d=4,c=2: 61 / 110 / 144
\item Soft Grudger: 62 / 109 / 142
\item Meta Majority Long Memory: 134 players: 63 / 62 / 62
\item Firm But Fair: 64 / 100 / 91
\item Level Punisher: 65 / 29 / 16
\item k68r: 66 / 117 / 139 / 12
\item k86r: 67 / 36 / 49 / 28
\item NMWE Long Memory: 134 players: 68 / 105 / 112
\item Meta Majority: 213 players: 69 / 66 / 75
\item ZD-GEN-2: 0.125, 0.5, 3: 70 / 99 / 110
\item k66r: 71 / 41 / 19 / 20
\item Evolved ANN 5 Noise 05: 72 / 12 / 2
\item Second by Eatherley: 73 / 64 / 79
\item k46r: 74 / 63 / 77 / 14
\item TF3: 75 / 75 / 90
\item Memory Decay: 0.1, 0.03, -2, 1, Tit For Tat, 15: 76 / 51 / 51
\item Nice Meta Winner: 213 players: 77 / 114 / 129
\item k72r: 78 / 77 / 38 / 13
\item k43r: 79 / 18 / 6 / 39
\item Doubler: 80 / 54 / 42
\item Meta Majority Finite Memory: 79 players: 81 / 59 / 64
\item GrudgerAlternator: 82 / 124 / 159
\item k34r: 83 / 111 / 119 / 52
\item k47r: 84 / 16 / 5 / 16
\item k61r: 85 / 126 / 156 / 2
\item Second by Champion: 86 / 108 / 93
\item k35r: 87 / 95 / 89 / 11
\item k79r: 88 / 52 / 54 / 26
\item k91r: 89 / 67 / 52 / 30
\item ShortMem: 90 / 56 / 32
\item Dynamic Two Tits For Tat: 91 / 94 / 92
\item k64r: 92 / 71 / 46 / 17
\item Adaptive Pavlov 2011: 93 / 112 / 121
\item First by Tideman and Chieruzzi: (D, D): 94 / 120 / 102
\item Adaptive Pavlov 2006: 95 / 113 / 131
\item Meta Majority Memory One: 36 players: 96 / 101 / 87
\item Once Bitten: 97 / 45 / 39
\item First by Davis: 10: 98 / 127 / 122
\item k53r: 99 / 128 / 128 / 45
\item Soft Go By Majority: 5: 100 / 50 / 35
\item k73r: 101 / 44 / 50 / 41
\item Limited Retaliate 3: 0.05, 20: 102 / 130 / 152
\item Inverse Punisher: 103 / 132 / 157
\item k70r: 104 / 129 / 149 / 32
\item Forgiver: 105 / 82 / 96
\item k83r: 106 / 92 / 83 / 15
\item Limited Retaliate 2: 0.08, 15: 107 / 134 / 164
\item Slow Tit For Two Tats 2: 108 / 68 / 74
\item First by Grofman: 109 / 135 / 176
\item k75r: 110 / 42 / 31 / 8
\item Stalker: (D,): 111 / 88 / 65
\item VeryBad: 112 / 89 / 60
\item k37r: 113 / 73 / 57 / 37
\item Hard Tit For 2 Tats: 114 / 83 / 70
\item k57r: 115 / 147 / 182 / 31
\item Soft Go By Majority: 10: 116 / 76 / 47
\item Soft Go By Majority: 20: 117 / 84 / 55
\item Soft Go By Majority: 40: 118 / 96 / 66
\item Limited Retaliate: 0.1, 20: 119 / 138 / 170
\item Nice Average Copier: 120 / 123 / 133
\item Worse and Worse 3: 121 / 125 / 132
\item Punisher: 122 / 137 / 167
\item Retaliate 2: 0.08: 123 / 139 / 163
\item Second by Appold: 124 / 119 / 106
\item Retaliate 3: 0.05: 125 / 133 / 153
\item k88r: 126 / 122 / 113 / 22
\item k31r: 127 / 107 / 73 / 23
\item Math Constant Hunter: 128 / 136 / 146
\item Forgetful Grudger: 129 / 144 / 172
\item k39r: 130 / 81 / 20 / 25
\item Retaliate: 0.1: 131 / 143 / 171
\item k90r: 132 / 104 / 71 / 24
\item Grumpy: Nice, 10, -10: 133 / 118 / 88
\item N Tit(s) For M Tat(s): 3, 2: 134 / 85 / 81
\item Thumper: 135 / 148 / 161
\item Two Tits For Tat: 136 / 146 / 165
\item Inverse: 137 / 140 / 148
\item Delayed AON1: 138 / 152 / 215
\item Hard Tit For Tat: 139 / 150 / 178
\item Tricky Level Punisher: 140 / 106 / 117
\item Appeaser: 141 / 155 / 205
\item Win-Stay Lose-Shift: 142 / 156 / 206
\item AdaptorBrief: 143 / 78 / 53
\item k69r: 144 / 121 / 48 / 29
\item k78r: 145 / 80 / 61 / 19
\item k67r: 146 / 103 / 33 / 27
\item Eventual Cycle Hunter: 147 / 157 / 198
\item k82r: 148 / 58 / 28 / 49
\item First by Nydegger: 149 / 153 / 173
\item First by Graaskamp: 0.05: 150 / 102 / 82
\item k48r: 151 / 141 / 94 / 53
\item Random Hunter: 152 / 154 / 154
\item UsuallyCooperates: 153 / 183 / 230
\item Cycle Hunter: 154 / 169 / 193
\item k76r: 155 / 166 / 155 / 46
\item Second by Tester: 156 / 163 / 151
\item Defector Hunter: 157 / 173 / 204
\item Raider: 158 / 161 / 134
\item Alternator Hunter: 159 / 175 / 200
\item AdaptorLong: 160 / 149 / 169
\item Ripoff: 161 / 172 / 162
\item Average Copier: 162 / 171 / 177
\item k45r: 163 / 159 / 115 / 50
\item k51r: 164 / 167 / 158 / 18
\item Prober 2: 165 / 162 / 130
\item k33r: 166 / 178 / 145 / 59
\item Knowledgeable Worse and Worse: 167 / 181 / 214
\item Cooperator: 168 / 179 / 211
\item k52r: 169 / 151 / 100 / 48
\item k77r: 170 / 131 / 45 / 55
\item Hard Prober: 171 / 164 / 125
\item Sneaky Tit For Tat: 172 / 180 / 179
\item k62r: 173 / 158 / 99 / 51
\item DoubleResurrection: 174 / 165 / 105
\item k89r: 175 / 200 / 191 / 56
\item Suspicious Tit For Tat: 176 / 185 / 160
\item Willing: 177 / 192 / 203
\item Remorseful Prober: 0.1: 178 / 168 / 114
\item First by Feld: 1.0, 0.5, 200: 179 / 145 / 84
\item First by Downing: 180 / 174 / 86
\item ZD-Mem2: 181 / 170 / 141
\item Worse and Worse 2: 182 / 142 / 98
\item Risky QLearner: 183 / 195 / 217
\item Cautious QLearner: 184 / 194 / 218
\item Arrogant QLearner: 185 / 196 / 216
\item Hesitant QLearner: 186 / 197 / 219
\item Detective: 187 / 189 / 166
\item Random Tit for Tat: 0.5: 188 / 188 / 180
\item First by Tullock: 189 / 160 / 116
\item k74r: 190 / 186 / 120 / 61
\item k54r: 191 / 191 / 143 / 58
\item Adaptive: 192 / 184 / 150
\item Worse and Worse: 193 / 190 / 212
\item Prober: 194 / 193 / 174
\item Hard Go By Majority: 5: 195 / 198 / 181
\item Hard Go By Majority: 196 / 202 / 194
\item Opposite Grudger: 197 / 208 / 236
\item Stochastic Cooperator: 198 / 187 / 187
\item Pun1: 199 / 206 / 199
\item Naive Prober: 0.1: 200 / 177 / 137
\item EasyGo: 201 / 220 / 259
\item First by Joss: 0.9: 202 / 176 / 136
\item ALLCorALLD: 203 / 211 / 228
\item Hard Go By Majority: 40: 204 / 201 / 188
\item Prober 4: 205 / 203 / 183
\item Prober 3: 206 / 199 / 175
\item Hard Go By Majority: 20: 207 / 207 / 185
\item Calculator: 208 / 182 / 135
\item Hard Go By Majority: 10: 209 / 209 / 186
\item SolutionB5: 210 / 210 / 184
\item Winner21: 211 / 221 / 225
\item Meta Mixer: 213 players: 212 / 205 / 195
\item Fortress3: 213 / 223 / 226
\item Fortress4: 214 / 224 / 222
\item Meta Hunter Aggressive: 7 players: 215 / 212 / 202
\item Cycler CCCCCD: 216 / 219 / 238
\item Stochastic WSLS: 0.05: 217 / 204 / 229
\item Cycler CCCDCD: 218 / 227 / 244
\item k71r: 219 / 222 / 220 / 60
\item Cycler CCCD: 220 / 228 / 245
\item ZD-SET-2: 0.25, 0.0, 2: 221 / 215 / 210
\item TF2: 222 / 229 / 231
\item Cooperator Hunter: 223 / 241 / 253
\item SelfSteem: 224 / 230 / 234
\item SolutionB1: 225 / 243 / 258
\item Cycler CCD: 226 / 231 / 239
\item Meta Winner Long Memory: 134 players: 227 / 216 / 189
\item Meta Winner: 213 players: 228 / 217 / 192
\item Alternator: 229 / 236 / 241
\item k63r: 230 / 240 / 248 / 57
\item Meta Winner Deterministic: 146 players: 231 / 218 / 190
\item ZD-Extort-2 v2: 0.125, 0.5, 1: 232 / 214 / 196
\item ZD-Extort-2: 0.1111111111111111, 0.5: 233 / 213 / 197
\item Meta Winner Ensemble: 213 players: 234 / 232 / 208
\item Meta Winner Stochastic: 67 players: 235 / 233 / 209
\item Win-Shift Lose-Stay: D: 236 / 244 / 247
\item Meta Winner Finite Memory: 79 players: 237 / 225 / 201
\item Cycler DC: 238 / 242 / 246
\item Meta Winner Memory One: 36 players: 239 / 234 / 207
\item k50r: 240 / 235 / 249 / 54
\item TF1: 241 / 238 / 224
\item ThueMorse: 242 / 250 / 256
\item Cycler DDC: 243 / 257 / 257
\item ZD-Extort3: 0.11538461538461539, 0.3333333333333333, 1: 244 / 226 / 213
\item AntiCycler: 245 / 259 / 263
\item Predator: 246 / 247 / 235
\item k36r: 247 / 251 / 243 / 63
\item ZD-Extort-4: 0.23529411764705882, 0.25, 1: 248 / 239 / 221
\item ThueMorseInverse: 249 / 248 / 251
\item CollectiveStrategy: 250 / 246 / 227
\item $\pi$: 251 / 260 / 264
\item UsuallyDefects: 252 / 249 / 237
\item Tricky Cooperator: 253 / 256 / 260
\item ZD-Mischief: 0.1, 0.0, 1: 254 / 237 / 223
\item Aggravater: 255 / 254 / 233
\item Better and Better: 256 / 258 / 242
\item ZD-Extortion: 0.2, 0.1, 1: 257 / 245 / 232
\item $e$: 258 / 261 / 265
\item First by Anonymous: 259 / 253 / 254
\item krandomc: 260 / 252 / 255 / 62
\item Bush Mosteller: 0.5, 0.5, 3.0, 0.5: 261 / 255 / 250
\item Desperate: 262 / 263 / 262
\item Gradual Killer: (D, D, D, D, D, C, C): 263 / 266 / 267
\item Meta Minority: 213 players: 264 / 268 / 268
\item Hopeless: 265 / 265 / 266
\item Bully: 266 / 269 / 269
\item Defector: 267 / 262 / 240
\item Handshake: 268 / 264 / 252
\item Tricky Defector: 269 / 267 / 261
\item $\phi$: 270 / 270 / 271
\item Negation: 271 / 271 / 270
\item Anti Tit For Tat: 272 / 272 / 272


==> assets/list_of_original_tournament_players.tex <==
\item k31r - Original rank: 23. Authored by Gail Grisell
\item k32r - Original rank: 10. Authored by Charles Kluepfel
\item k33r - Original rank: 59. Authored by Harold Rabbie
\item k34r - Original rank: 52. Authored by James W Friedman
\item k35r - Original rank: 11. Authored by Abraham Getzler
\item k36r - Original rank: 63. Authored by Roger Hotz
\item k37r - Original rank: 37. Authored by George Lefevre
\item k38r - Original rank: 34. Authored by Nelson Weiderman
\item k39r - Original rank: 25. Authored by Tom Almy
\item k40r - Original rank: 35. Authored by Robert Adams
\item k41r - Original rank: 7. Authored by Herb Weiner
\item k42r - Original rank: 3. Authored by Otto Borufsen
\item k43r - Original rank: 39. Authored by R D Anderson
\item k44r - Original rank: 5. Authored by William Adams
\item k45r - Original rank: 50. Authored by Michael F McGurrin
\item k46r - Original rank: 14. Authored by Graham J Eatherley
\item k47r - Original rank: 16. Authored by Richard Hufford
\item k48r - Original rank: 53. Authored by George Hufford
\item k49r - Original rank: 4. Authored by Rob Cave
\item k50r - Original rank: 54. Authored by Rik Smoody
\item k51r - Original rank: 18. Authored by John William Colbert
\item k52r - Original rank: 48. Authored by David A Smith
\item k53r - Original rank: 45. Authored by Henry Nussbacher
\item k54r - Original rank: 58. Authored by William H Robertson
\item k55r - Original rank: 42. Authored by Steve Newman
\item k56r - Original rank: 38. Authored by Stanley F Quayle
\item k57r - Original rank: 31. Authored by Rudy Nydegger
\item k58r - Original rank: 21. Authored by Glen Rowsam
\item k59r - Original rank: 40. Authored by Leslie Downing
\item k60r - Original rank: 6. Authored by Jim Graaskamp and Ken Katzen
\item k61r - Original rank: 2. Authored by Danny C Champion
\item k62r - Original rank: 51. Authored by Howard R Hollander
\item k63r - Original rank: 57. Authored by George Duisman
\item k64r - Original rank: 17. Authored by Brian Yamachi
\item k65r - Original rank: 47. Authored by Mark F Batell
\item k66r - Original rank: 20. Authored by Ray Mikkelson
\item k67r - Original rank: 27. Authored by Craig Feathers
\item k68r - Original rank: 12. Authored by Fransois Leyvraz
\item k69r - Original rank: 29. Authored by Johann Joss
\item k70r - Original rank: 32. Authored by Robert Pebly
\item k71r - Original rank: 60. Authored by James E Hall
\item k72r - Original rank: 13. Authored by Edward C White Jr
\item k73r - Original rank: 41. Authored by George Zimmerman
\item k74r - Original rank: 61. Authored by Edward Friedland
\item k75r - Original rank: 8. Authored by Paul D Harrington
\item k76r - Original rank: 46. Authored by David Gladstein
\item k77r - Original rank: 55. Authored by Scott Feld
\item k78r - Original rank: 19. Authored by Fred Mauk
\item k79r - Original rank: 26. Authored by Dennis Ambuehl and Kevin Hickey
\item k80r - Original rank: 36. Authored by Robyn M Dawes and Mark Batell
\item k81r - Original rank: 43. Authored by Martyn Jones
\item k82r - Original rank: 49. Authored by Robert A Leyland
\item k83r - Original rank: 15. Authored by Paul E Black
\item k84r - Original rank: 9. Authored by T Nicolaus Tideman and Paula Chieruzz
\item k85r - Original rank: 33. Authored by Robert B Falk and James M Langsted
\item k86r - Original rank: 28. Authored by Bernard Grofman
\item k87r - Original rank: 44. Authored by E E H Schurmann
\item k88r - Original rank: 22. Authored by Scott Appold
\item k89r - Original rank: 56. Authored by Gene Snodgrass
\item k90r - Original rank: 24. Authored by John Maynard Smith
\item k91r - Original rank: 30. Authored by Jonathan Pinkley
\item k92r - Original rank: 1. Authored by Anatol Rapoport
\item krandomc - Original rank: 62. Authored by None


==> assets/noisy_tournament_overall_cooperation_rate_in_1_percent_noise.tex <==
0.597

==> assets/noisy_tournament_overall_cooperation_rate_in_5_percent_noise.tex <==
0.51

==> assets/noisy_tournament_rankings_in_1_percent_noise.tex <==
\begin{tabular}{lrrrrrrr}
\toprule
 & Mean Score & Rank & Coop. Rate & Original Rank & Reproduced Coop. Rate & Library Rank & Library Coop. Rate \\
\midrule
Evolved FSM 16 Noise 05\textsuperscript{\textdagger} & 2.699 & 1 & 0.680 & NA & NA & 6 & 0.717 \\
DBS: 0.75, 3, 4, 3, 5 & 2.670 & 2 & 0.731 & NA & NA & 11 & 0.739 \\
Evolved ANN\textsuperscript{\textdagger} & 2.658 & 3 & 0.731 & NA & NA & 5 & 0.727 \\
Omega TFT: 3, 8 & 2.652 & 4 & 0.682 & NA & NA & 12 & 0.725 \\
k65r & 2.651 & 5 & 0.611 & 47 & 0.715 & NA & NA \\
k81r & 2.648 & 6 & 0.634 & 43 & 0.779 & NA & NA \\
Evolved ANN 5\textsuperscript{\textdagger} & 2.642 & 7 & 0.671 & NA & NA & 3 & 0.713 \\
BackStabber: (D, D) & 2.641 & 8 & 0.654 & NA & NA & 18 & 0.641 \\
PSO Gambler 2\_2\_2 Noise 05\textsuperscript{\textdagger} & 2.640 & 9 & 0.647 & NA & NA & 14 & 0.723 \\
k80r & 2.625 & 10 & 0.722 & 36 & 0.809 & NA & NA \\
DoubleCrosser: (D, D) & 2.625 & 11 & 0.690 & NA & NA & 13 & 0.677 \\
Evolved ANN 5 Noise 05\textsuperscript{\textdagger} & 2.623 & 12 & 0.714 & NA & NA & 45 & 0.544 \\
Evolved HMM 5\textsuperscript{\textdagger} & 2.622 & 13 & 0.621 & NA & NA & 2 & 0.742 \\
Fool Me Once & 2.618 & 14 & 0.556 & NA & NA & 17 & 0.624 \\
Evolved FSM 16\textsuperscript{\textdagger} & 2.616 & 15 & 0.647 & NA & NA & 4 & 0.713 \\
k47r & 2.611 & 16 & 0.613 & 16 & 0.723 & NA & NA \\
Gradual & 2.608 & 17 & 0.723 & NA & NA & 15 & 0.793 \\
k43r & 2.607 & 18 & 0.643 & 39 & 0.667 & NA & NA \\
Forgetful Fool Me Once: 0.05 & 2.606 & 19 & 0.686 & NA & NA & 20 & 0.753 \\
Original Gradual & 2.602 & 20 & 0.778 & NA & NA & NA & NA \\
k56r & 2.602 & 21 & 0.710 & 38 & 0.891 & NA & NA \\
Revised Downing & 2.601 & 22 & 0.710 & NA & NA & NA & NA \\
k59r & 2.601 & 23 & 0.710 & 40 & 0.892 & NA & NA \\
Spiteful Tit For Tat & 2.600 & 24 & 0.590 & NA & NA & 19 & 0.664 \\
k42r & 2.600 & 25 & 0.767 & 3 & 0.916 & NA & NA \\
\bottomrule
\end{tabular}


==> assets/noisy_tournament_rankings_in_5_percent_noise.tex <==
\begin{tabular}{lrrrrrrr}
\toprule
 & Mean Score & Rank & Coop. Rate & Original Rank & Reproduced Coop. Rate & Library Rank & Library Coop. Rate \\
\midrule
DBS: 0.75, 3, 4, 3, 5 & 2.510 & 1 & 0.567 & NA & NA & 11 & 0.739 \\
Evolved ANN 5 Noise 05\textsuperscript{\textdagger} & 2.480 & 2 & 0.648 & NA & NA & 45 & 0.544 \\
k80r & 2.461 & 3 & 0.623 & 36 & 0.809 & NA & NA \\
Evolved FSM 16 Noise 05\textsuperscript{\textdagger} & 2.456 & 4 & 0.526 & NA & NA & 6 & 0.717 \\
k47r & 2.449 & 5 & 0.492 & 16 & 0.723 & NA & NA \\
k43r & 2.448 & 6 & 0.560 & 39 & 0.667 & NA & NA \\
k38r & 2.433 & 7 & 0.622 & 34 & 0.874 & NA & NA \\
Evolved ANN\textsuperscript{\textdagger} & 2.430 & 8 & 0.577 & NA & NA & 5 & 0.727 \\
BackStabber: (D, D) & 2.426 & 9 & 0.458 & NA & NA & 18 & 0.641 \\
Revised Downing & 2.421 & 10 & 0.512 & NA & NA & NA & NA \\
k59r & 2.420 & 11 & 0.512 & 40 & 0.892 & NA & NA \\
k56r & 2.419 & 12 & 0.511 & 38 & 0.891 & NA & NA \\
DoubleCrosser: (D, D) & 2.415 & 13 & 0.529 & NA & NA & 13 & 0.677 \\
k81r & 2.406 & 14 & 0.469 & 43 & 0.779 & NA & NA \\
k55r & 2.403 & 15 & 0.528 & 42 & 0.903 & NA & NA \\
Level Punisher & 2.400 & 16 & 0.567 & NA & NA & 44 & 0.731 \\
Omega TFT: 3, 8 & 2.399 & 17 & 0.502 & NA & NA & 12 & 0.725 \\
k65r & 2.397 & 18 & 0.387 & 47 & 0.715 & NA & NA \\
k66r & 2.389 & 19 & 0.679 & 20 & 0.866 & NA & NA \\
k39r & 2.378 & 20 & 0.619 & 25 & 0.676 & NA & NA \\
k42r & 2.376 & 21 & 0.637 & 3 & 0.916 & NA & NA \\
Spiteful Tit For Tat & 2.373 & 22 & 0.388 & NA & NA & 19 & 0.664 \\
k49r & 2.366 & 23 & 0.696 & 4 & 0.892 & NA & NA \\
PSO Gambler 2\_2\_2 Noise 05\textsuperscript{\textdagger} & 2.363 & 24 & 0.515 & NA & NA & 14 & 0.723 \\
k60r & 2.357 & 25 & 0.439 & 6 & 0.844 & NA & NA \\
\bottomrule
\end{tabular}


==> assets/number_of_extra_strategy_repetitions.tex <==
12500

==> assets/number_of_full_repetitions.tex <==
25,000

==> assets/number_of_full_repetitions_in_1_percent_noise_tournament.tex <==
3,250

==> assets/number_of_full_repetitions_in_5_percent_noise_tournament.tex <==
1,750

==> assets/number_of_sp_repetitions.tex <==
30000

==> assets/number_of_strategies_in_1_percent_noise_tournament.tex <==
272

==> assets/number_of_strategies_in_5_percent_noise_tournament.tex <==
272

==> assets/number_of_translated_strategies.tex <==
28

==> assets/original_strategies_rankings.tex <==
\begin{tabular}{lccccccc}
\toprule
 & \makecell[c]{Original\\Rank} & \makecell[c]{Reproduced\\Rank} & \makecell[c]{Reproduced Rank\\(Noise 1\%)} & \makecell[c]{S \& P\\tournament Rank} & \makecell[c]{AXL\\tournament Rank} & \makecell[c]{AXL (Noise 1\%)\\tournament Rank} & \makecell[c]{AXL (Noise 5\%)\\tournament Rank} \\
\midrule
k92r & 1 & 1 & 28 & 4 & 57 & 70 & 69 \\
k61r & 2 & 12 & 44 & 8 & 85 & 126 & 156 \\
k42r & 3 & 2 & 8 & 2 & 16 & 25 & 21 \\
k49r & 4 & 4 & 12 & 5 & 30 & 32 & 23 \\
k44r & 5 & 3 & 16 & 7 & 46 & 37 & 26 \\
k60r & 6 & 9 & 11 & 16 & 19 & 31 & 25 \\
k41r & 7 & 8 & 13 & 10 & 35 & 33 & 40 \\
k75r & 8 & 5 & 20 & 6 & 110 & 42 & 31 \\
k84r & 9 & 7 & 21 & 15 & 47 & 43 & 76 \\
k32r & 10 & 6 & 18 & 12 & 23 & 40 & 34 \\
k35r & 11 & 11 & 36 & 14 & 87 & 95 & 89 \\
k68r & 12 & 10 & 41 & 9 & 66 & 117 & 139 \\
k72r & 13 & 13 & 32 & 13 & 78 & 77 & 38 \\
k46r & 14 & 14 & 26 & 11 & 74 & 63 & 77 \\
k83r & 15 & 15 & 35 & 17 & 106 & 92 & 83 \\
k47r & 16 & 16 & 4 & 22 & 84 & 16 & 5 \\
k64r & 17 & 17 & 29 & 18 & 92 & 71 & 46 \\
k51r & 18 & 19 & 54 & 30 & 164 & 167 & 158 \\
k78r & 19 & 20 & 33 & 37 & 145 & 80 & 61 \\
k66r & 20 & 18 & 19 & 19 & 71 & 41 & 19 \\
k58r & 21 & 21 & 17 & 23 & 25 & 38 & 43 \\
k88r & 22 & 22 & 43 & 25 & 126 & 122 & 113 \\
k31r & 23 & 23 & 39 & 24 & 127 & 107 & 73 \\
k90r & 24 & 26 & 38 & 27 & 132 & 104 & 71 \\
k39r & 25 & 27 & 34 & 21 & 130 & 81 & 20 \\
k79r & 26 & 24 & 23 & 26 & 88 & 52 & 54 \\
k67r & 27 & 25 & 37 & 28 & 146 & 103 & 33 \\
k86r & 28 & 30 & 15 & 33 & 67 & 36 & 49 \\
k69r & 29 & 31 & 42 & 43 & 144 & 121 & 48 \\
k91r & 30 & 28 & 27 & 29 & 89 & 67 & 52 \\
k57r & 31 & 29 & 49 & 40 & 115 & 147 & 182 \\
k70r & 32 & 35 & 46 & 41 & 104 & 129 & 149 \\
k85r & 33 & 37 & 24 & 47 & 20 & 57 & 101 \\
k38r & 34 & 33 & 9 & 34 & 51 & 26 & 7 \\
k40r & 35 & 32 & 14 & 38 & 27 & 34 & 80 \\
k80r & 36 & 34 & 3 & 31 & 22 & 10 & 3 \\
k37r & 37 & 42 & 30 & 44 & 113 & 73 & 57 \\
k56r & 38 & 41 & 6 & 36 & 31 & 21 & 12 \\
k43r & 39 & 38 & 5 & 32 & 79 & 18 & 6 \\
k59r & 40 & 40 & 7 & 35 & 32 & 23 & 11 \\
k73r & 41 & 44 & 22 & 42 & 101 & 44 & 50 \\
k55r & 42 & 43 & 10 & 39 & 36 & 27 & 15 \\
k81r & 43 & 45 & 2 & 45 & 43 & 6 & 14 \\
k87r & 44 & 39 & 31 & 46 & 26 & 74 & 124 \\
k53r & 45 & 46 & 45 & 49 & 99 & 128 & 128 \\
k76r & 46 & 36 & 53 & 48 & 155 & 166 & 155 \\
k65r & 47 & 48 & 1 & 50 & 28 & 5 & 18 \\
k52r & 48 & 47 & 50 & 51 & 169 & 151 & 100 \\
k82r & 49 & 50 & 25 & 56 & 148 & 58 & 28 \\
k45r & 50 & 49 & 52 & 55 & 163 & 159 & 115 \\
k62r & 51 & 51 & 51 & 57 & 173 & 158 & 99 \\
k34r & 52 & 52 & 40 & 58 & 83 & 111 & 119 \\
k48r & 53 & 53 & 48 & 60 & 151 & 141 & 94 \\
k50r & 54 & 54 & 60 & 62 & 240 & 235 & 249 \\
k77r & 55 & 55 & 47 & 64 & 170 & 131 & 45 \\
k89r & 56 & 56 & 58 & 63 & 175 & 200 & 191 \\
k63r & 57 & 58 & 61 & 67 & 230 & 240 & 248 \\
k54r & 58 & 57 & 57 & 65 & 191 & 191 & 143 \\
k33r & 59 & 59 & 55 & 66 & 166 & 178 & 145 \\
k71r & 60 & 60 & 59 & 68 & 219 & 222 & 220 \\
k74r & 61 & 61 & 56 & 69 & 190 & 186 & 120 \\
krandomc & 62 & 62 & 63 & 71 & 260 & 252 & 255 \\
k36r & 63 & 63 & 62 & 72 & 247 & 251 & 243 \\
\bottomrule
\end{tabular}


==> assets/original_tournament_overall_cooperation_rate.tex <==
0.750

==> assets/original_tournament_predictive_12_model.tex <==
\begin{tabular}{lrll}
\toprule
Strategies &  Coefficients &    $p$-value & $F$-value \\
\midrule
      k31r &         0.166 &  5.15065e-05 &   18.9782 \\
      k34r &         0.081 &  1.39931e-08 &   42.8242 \\
      k51r &         0.230 &   0.00357868 &    9.1841 \\
      k52r &         0.116 &     0.572461 &   0.32205 \\
      k56r &        -1.695 &   1.2278e-09 &   51.2719 \\
      k59r &         1.729 &   1.2399e-09 &   51.2364 \\
      k64r &        -0.150 &  2.41824e-14 &   98.4147 \\
      k79r &         0.121 &  2.36814e-14 &   98.5231 \\
      k82r &         0.120 &  1.08815e-06 &   29.3393 \\
      k84r &         0.220 &  9.37609e-18 &   144.822 \\
      k88r &         0.112 &   1.8614e-15 &   112.266 \\
      k91r &         0.066 &  2.50396e-10 &   57.1748 \\
 Intercept &        -0.485 &           NA &        NA \\
\bottomrule
\end{tabular}


==> assets/original_tournament_predictive_12_r_squared.tex <==
0.9840

==> assets/original_tournament_predictive_17_model.tex <==
\begin{tabular}{lrll}
\toprule
Strategies & Coefficients & $p$-value & $F$-value \\
\midrule
k32r & -0.114000 & 0.000000 & 186.247539 \\
k36r & 0.183000 & 0.189994 & 1.756582 \\
k41r & 0.098000 & 0.000000 & 177.937911 \\
k42r & 0.113000 & 0.000000 & 79.351204 \\
k48r & 0.044000 & 0.007426 & 7.670719 \\
k51r & 0.090000 & 0.002438 & 10.001032 \\
k56r & -4.540000 & 0.000000 & 48.729856 \\
k59r & 4.615000 & 0.000000 & 48.744926 \\
k62r & 0.066000 & 0.703116 & 0.146621 \\
k66r & 0.100000 & 0.000000 & 135.614172 \\
k70r & 0.098000 & 0.000000 & 79.384616 \\
k73r & 0.112000 & 0.000000 & 67.006588 \\
k76r & 0.038000 & 0.025992 & 5.207451 \\
k82r & 0.035000 & 0.000001 & 29.385307 \\
k89r & 0.054000 & 0.015430 & 6.210811 \\
k90r & 0.028000 & 0.960298 & 0.002498 \\
k91r & 0.062000 & 0.000000 & 56.667196 \\
Intercept & -0.025000 & NA & NA \\
\bottomrule
\end{tabular}


==> assets/original_tournament_predictive_17_r_squared.tex <==
0.9966

==> assets/original_tournament_predictive_25_model.tex <==
\begin{tabular}{lrll}
\toprule
Strategies & Coefficients & $p$-value & $F$-value \\
\midrule
k31r & 0.062010 & 0.000079 & 17.918667 \\
k33r & 0.016510 & 0.040154 & 4.397057 \\
k34r & 0.064100 & 0.000000 & 42.866846 \\
k35r & 0.062600 & 0.000000 & 89.112013 \\
k37r & 0.037950 & 0.000000 & 124.456685 \\
k43r & 0.022480 & 0.000000 & 97.073236 \\
k47r & 0.042120 & 0.000000 & 43.355694 \\
k48r & 0.022550 & 0.007426 & 7.670719 \\
k50r & 0.017440 & 0.000001 & 30.733454 \\
k52r & 0.061160 & 0.560299 & 0.342938 \\
k53r & -0.046330 & 0.000000 & 43.066908 \\
k54r & 0.018600 & 0.618827 & 0.250067 \\
k55r & 0.039250 & 0.000000 & 35.594335 \\
k66r & 0.027550 & 0.000000 & 135.614172 \\
k70r & 0.051980 & 0.000000 & 79.384616 \\
k75r & 0.021190 & 0.169382 & 1.933926 \\
k76r & 0.029890 & 0.025992 & 5.207451 \\
k77r & 0.035220 & 0.000351 & 14.339773 \\
k78r & 0.024600 & 0.000001 & 29.608895 \\
k83r & 0.118540 & 0.000001 & 28.599394 \\
k84r & 0.092840 & 0.000000 & 151.870987 \\
k85r & 0.050790 & 0.000000 & 79.165825 \\
k86r & 0.052540 & 0.000000 & 120.051625 \\
k89r & 0.017050 & 0.015430 & 6.210811 \\
krandomc & 0.031560 & 0.790835 & 0.070965 \\
Intercept & 0.017800 & NA & NA \\
\bottomrule
\end{tabular}


==> assets/original_tournament_predictive_25_r_squared.tex <==
0.999

==> assets/original_tournament_predictive_5_model.tex <==
\begin{tabular}{lrll}
\toprule
Strategies & Coefficients & $p$-value & $F$-value \\
\midrule
k31r & 0.090670 & 0.000079 & 17.918667 \\
k75r & 0.153570 & 0.169382 & 1.933926 \\
k83r & 0.407720 & 0.000001 & 28.599394 \\
k84r & 0.224340 & 0.000000 & 151.870987 \\
k85r & 0.159700 & 0.000000 & 79.165825 \\
Intercept & -0.336500 & NA & NA \\
\bottomrule
\end{tabular}


==> assets/original_tournament_predictive_5_r_squared.tex <==
0.952

==> assets/original_tournament_predictive_8_model.tex <==
\begin{tabular}{lrll}
\toprule
Strategies & Coefficients & $p$-value & $F$-value \\
\midrule
k31r & 0.114690 & 0.000079 & 17.918667 \\
k52r & 0.053740 & 0.560299 & 0.342938 \\
k75r & 0.076090 & 0.169382 & 1.933926 \\
k76r & 0.054960 & 0.025992 & 5.207451 \\
k77r & 0.054520 & 0.000351 & 14.339773 \\
k83r & 0.288080 & 0.000001 & 28.599394 \\
k84r & 0.210160 & 0.000000 & 151.870987 \\
k85r & 0.181210 & 0.000000 & 79.165825 \\
Intercept & -0.229290 & NA & NA \\
\bottomrule
\end{tabular}


==> assets/original_tournament_predictive_8_r_squared.tex <==
0.981

==> assets/original_tournament_predictive_with_axelrod_5_model.tex <==
\begin{tabular}{lrll}
\toprule
Strategies & Coefficients & $p$-value & $F$-value \\
\midrule
k60r & 0.232010 & 0.000000 & 298.163936 \\
k91r & 0.187930 & 0.000000 & 56.667196 \\
k40r & 0.071870 & 0.000000 & 78.191831 \\
k76r & 0.063670 & 0.025992 & 5.207451 \\
k67r & 0.113650 & 0.000002 & 27.893148 \\
Intercept & 0.790880 & NA & NA \\
\bottomrule
\end{tabular}


==> assets/original_tournament_representative_model.tex <==
\begin{tabular}{lr}
\toprule
Strategies & Coefficients \\
\midrule
k60r & 0.202000 \\
k91r & 0.198000 \\
k40r & 0.110000 \\
k76r & 0.072000 \\
k67r & 0.086000 \\
Intercept & 0.795000 \\
\bottomrule
\end{tabular}


==> assets/original_tournament_representative_r_squared.tex <==
0.9517

==> assets/original_tournament_with_extra_strategy_summary.tex <==
\begin{tabular}{lrrl}
\toprule
 & Mean Score & Rank & Winner \\
Name &  &  &  \\
\midrule
Adaptive Tit For Tat: 0.5 & 2.876 & 2 & k92r \\
GTFT: 0.33 & 2.846 & 3 & k92r \\
Omega TFT: 3, 8 & 2.859 & 3 & k92r \\
Firm But Fair & 2.861 & 3 & k92r \\
ZD-GTFT-2: 0.25, 0.5 & 2.868 & 3 & k92r \\
Resurrection & 2.867 & 3 & k92r \\
Meta Majority: 213 players & 2.860 & 3 & k92r \\
Meta Majority Finite Memory: 79 players & 2.856 & 3 & k92r \\
Meta Majority Long Memory: 134 players & 2.856 & 3 & k92r \\
Soft Joss: 0.9 & 2.871 & 3 & k92r \\
Forgiving Tit For Tat & 2.854 & 3 & k92r \\
Original Gradual & 2.857 & 3 & k92r \\
Meta Majority Memory One: 36 players & 2.838 & 4 & k92r \\
PSO Gambler 2\_2\_2 Noise 05\textsuperscript{\textdagger} & 2.840 & 4 & k92r \\
Gradual & 2.831 & 7 & k92r \\
First by Stein and Rapoport: 0.05: (D, D) & 2.827 & 8 & k92r \\
Spiteful Tit For Tat & 2.826 & 8 & k92r \\
GrudgerAlternator & 2.825 & 8 & k92r \\
EugineNier: (D,) & 2.815 & 10 & k92r \\
First by Shubik & 2.791 & 13 & k92r \\
\bottomrule
\end{tabular}


==> assets/original_tournament_with_trained_strategy.tex <==
\begin{tabular}{lrrrrl}
\toprule
{} &  Cooperation Rate against opponents &  Cooperation Rate from opponents &  Rank &  Score &            Winner \\
Training environment                 &                                     &                                  &       &        &                   \\
\midrule
Full Players                         &                               0.919 &                            0.917 &     1 &  2.933 &  Trained strategy \\
Full Players With Axl                &                               0.946 &                            0.919 &     2 &  2.839 &              k92r \\
Predictive 5 Strategies              &                               0.790 &                            0.746 &    41 &  2.621 &              k92r \\
Representative Strategies            &                               0.599 &                            0.652 &    52 &  2.479 &              k92r \\
Predictive 12 Strategies             &                               0.758 &                            0.656 &    53 &  2.423 &              k92r \\
Predictive With Axelrod 5 Strategies &                               0.777 &                            0.687 &    53 &  2.384 &              k92r \\
\bottomrule
\end{tabular}


==> assets/si_list_of_all_strategies.tex <==
\item EvolvedLookerUp2_2_2: 1 / 30 / 118
\item Evolved HMM 5: 2 / 13 / 59
\item Omega TFT: 3, 8: 3 / 4 / 17
\item Evolved ANN 5: 4 / 7 / 36
\item Evolved ANN: 5 / 3 / 8
\item Evolved FSM 16: 6 / 15 / 78
\item Evolved FSM 16 Noise 05: 7 / 1 / 4
\item PSO Gambler 2_2_2: 8 / 53 / 138
\item Original Gradual: 9 / 20 / 30
\item PSO Gambler 2_2_2 Noise 05: 10 / 9 / 24
\item PSO Gambler Mem1: 11 / 39 / 107
\item Evolved FSM 4: 12 / 28 / 85
\item PSO Gambler 1_1_1: 13 / 61 / 140
\item Gradual: 14 / 17 / 29
\item DBS: 0.75, 3, 4, 3, 5: 15 / 2 / 1
\item k42r: 16 / 25 / 21 / 3
\item Winner12: 17 / 60 / 127
\item Spiteful Tit For Tat: 18 / 24 / 22
\item k60r: 19 / 31 / 25 / 6
\item k85r: 20 / 57 / 101 / 33
\item EugineNier: (D,): 21 / 35 / 27
\item k80r: 22 / 10 / 3 / 36
\item k32r: 23 / 40 / 34 / 10
\item DoubleCrosser: (D, D): 24 / 11 / 13
\item k58r: 25 / 38 / 43 / 21
\item k87r: 26 / 74 / 124 / 44
\item k40r: 27 / 34 / 80 / 35
\item k65r: 28 / 5 / 18 / 47
\item Forgetful Fool Me Once: 0.05: 29 / 19 / 41
\item k49r: 30 / 32 / 23 / 4
\item k56r: 31 / 21 / 12 / 38
\item k59r: 32 / 23 / 11 / 40
\item Revised Downing: 33 / 22 / 10
\item Fool Me Once: 34 / 14 / 37
\item k41r: 35 / 33 / 40 / 7
\item k55r: 36 / 27 / 15 / 42
\item First by Shubik: 37 / 87 / 95
\item ZD-GTFT-2: 0.25, 0.5: 38 / 48 / 63
\item Soft Joss: 0.9: 39 / 49 / 56
\item BackStabber: (D, D): 40 / 8 / 9
\item MEM2: 41 / 79 / 103
\item AON2: 42 / 116 / 168
\item k81r: 43 / 6 / 14 / 43
\item Meta Hunter: 6 players: 44 / 69 / 108
\item NMWE Finite Memory: 79 players: 45 / 91 / 126
\item k44r: 46 / 37 / 26 / 5
\item k84r: 47 / 43 / 76 / 9
\item GTFT: 0.33: 48 / 55 / 72
\item EvolvedLookerUp1_1_1: 49 / 115 / 147
\item NMWE Stochastic: 67 players: 50 / 97 / 123
\item k38r: 51 / 26 / 7 / 34
\item Michaelos: (D,): 52 / 86 / 97
\item First by Stein and Rapoport: 0.05: (D, D): 53 / 47 / 44
\item NMWE Memory One: 36 players: 54 / 90 / 104
\item Resurrection: 55 / 65 / 67
\item Nice Meta Winner Ensemble: 213 players: 56 / 98 / 111
\item k92r: 57 / 70 / 69 / 1
\item Adaptive Tit For Tat: 0.5: 58 / 72 / 68
\item Forgiving Tit For Tat: 59 / 46 / 58
\item NMWE Deterministic: 146 players: 60 / 93 / 109
\item General Soft Grudger: n=1,d=4,c=2: 61 / 110 / 144
\item Soft Grudger: 62 / 109 / 142
\item Meta Majority Long Memory: 134 players: 63 / 62 / 62
\item Firm But Fair: 64 / 100 / 91
\item Level Punisher: 65 / 29 / 16
\item k68r: 66 / 117 / 139 / 12
\item k86r: 67 / 36 / 49 / 28
\item NMWE Long Memory: 134 players: 68 / 105 / 112
\item Meta Majority: 213 players: 69 / 66 / 75
\item ZD-GEN-2: 0.125, 0.5, 3: 70 / 99 / 110
\item k66r: 71 / 41 / 19 / 20
\item Evolved ANN 5 Noise 05: 72 / 12 / 2
\item Second by Eatherley: 73 / 64 / 79
\item k46r: 74 / 63 / 77 / 14
\item TF3: 75 / 75 / 90
\item Memory Decay: 0.1, 0.03, -2, 1, Tit For Tat, 15: 76 / 51 / 51
\item Nice Meta Winner: 213 players: 77 / 114 / 129
\item k72r: 78 / 77 / 38 / 13
\item k43r: 79 / 18 / 6 / 39
\item Doubler: 80 / 54 / 42
\item Meta Majority Finite Memory: 79 players: 81 / 59 / 64
\item GrudgerAlternator: 82 / 124 / 159
\item k34r: 83 / 111 / 119 / 52
\item k47r: 84 / 16 / 5 / 16
\item k61r: 85 / 126 / 156 / 2
\item Second by Champion: 86 / 108 / 93
\item k35r: 87 / 95 / 89 / 11
\item k79r: 88 / 52 / 54 / 26
\item k91r: 89 / 67 / 52 / 30
\item ShortMem: 90 / 56 / 32
\item Dynamic Two Tits For Tat: 91 / 94 / 92
\item k64r: 92 / 71 / 46 / 17
\item Adaptive Pavlov 2011: 93 / 112 / 121
\item First by Tideman and Chieruzzi: (D, D): 94 / 120 / 102
\item Adaptive Pavlov 2006: 95 / 113 / 131
\item Meta Majority Memory One: 36 players: 96 / 101 / 87
\item Once Bitten: 97 / 45 / 39
\item First by Davis: 10: 98 / 127 / 122
\item k53r: 99 / 128 / 128 / 45
\item Soft Go By Majority: 5: 100 / 50 / 35
\item k73r: 101 / 44 / 50 / 41
\item Limited Retaliate 3: 0.05, 20: 102 / 130 / 152
\item Inverse Punisher: 103 / 132 / 157
\item k70r: 104 / 129 / 149 / 32
\item Forgiver: 105 / 82 / 96
\item k83r: 106 / 92 / 83 / 15
\item Limited Retaliate 2: 0.08, 15: 107 / 134 / 164
\item Slow Tit For Two Tats 2: 108 / 68 / 74
\item First by Grofman: 109 / 135 / 176
\item k75r: 110 / 42 / 31 / 8
\item Stalker: (D,): 111 / 88 / 65
\item VeryBad: 112 / 89 / 60
\item k37r: 113 / 73 / 57 / 37
\item Hard Tit For 2 Tats: 114 / 83 / 70
\item k57r: 115 / 147 / 182 / 31
\item Soft Go By Majority: 10: 116 / 76 / 47
\item Soft Go By Majority: 20: 117 / 84 / 55
\item Soft Go By Majority: 40: 118 / 96 / 66
\item Limited Retaliate: 0.1, 20: 119 / 138 / 170
\item Nice Average Copier: 120 / 123 / 133
\item Worse and Worse 3: 121 / 125 / 132
\item Punisher: 122 / 137 / 167
\item Retaliate 2: 0.08: 123 / 139 / 163
\item Second by Appold: 124 / 119 / 106
\item Retaliate 3: 0.05: 125 / 133 / 153
\item k88r: 126 / 122 / 113 / 22
\item k31r: 127 / 107 / 73 / 23
\item Math Constant Hunter: 128 / 136 / 146
\item Forgetful Grudger: 129 / 144 / 172
\item k39r: 130 / 81 / 20 / 25
\item Retaliate: 0.1: 131 / 143 / 171
\item k90r: 132 / 104 / 71 / 24
\item Grumpy: Nice, 10, -10: 133 / 118 / 88
\item N Tit(s) For M Tat(s): 3, 2: 134 / 85 / 81
\item Thumper: 135 / 148 / 161
\item Two Tits For Tat: 136 / 146 / 165
\item Inverse: 137 / 140 / 148
\item Delayed AON1: 138 / 152 / 215
\item Hard Tit For Tat: 139 / 150 / 178
\item Tricky Level Punisher: 140 / 106 / 117
\item Appeaser: 141 / 155 / 205
\item Win-Stay Lose-Shift: 142 / 156 / 206
\item AdaptorBrief: 143 / 78 / 53
\item k69r: 144 / 121 / 48 / 29
\item k78r: 145 / 80 / 61 / 19
\item k67r: 146 / 103 / 33 / 27
\item Eventual Cycle Hunter: 147 / 157 / 198
\item k82r: 148 / 58 / 28 / 49
\item First by Nydegger: 149 / 153 / 173
\item First by Graaskamp: 0.05: 150 / 102 / 82
\item k48r: 151 / 141 / 94 / 53
\item Random Hunter: 152 / 154 / 154
\item UsuallyCooperates: 153 / 183 / 230
\item Cycle Hunter: 154 / 169 / 193
\item k76r: 155 / 166 / 155 / 46
\item Second by Tester: 156 / 163 / 151
\item Defector Hunter: 157 / 173 / 204
\item Raider: 158 / 161 / 134
\item Alternator Hunter: 159 / 175 / 200
\item AdaptorLong: 160 / 149 / 169
\item Ripoff: 161 / 172 / 162
\item Average Copier: 162 / 171 / 177
\item k45r: 163 / 159 / 115 / 50
\item k51r: 164 / 167 / 158 / 18
\item Prober 2: 165 / 162 / 130
\item k33r: 166 / 178 / 145 / 59
\item Knowledgeable Worse and Worse: 167 / 181 / 214
\item Cooperator: 168 / 179 / 211
\item k52r: 169 / 151 / 100 / 48
\item k77r: 170 / 131 / 45 / 55
\item Hard Prober: 171 / 164 / 125
\item Sneaky Tit For Tat: 172 / 180 / 179
\item k62r: 173 / 158 / 99 / 51
\item DoubleResurrection: 174 / 165 / 105
\item k89r: 175 / 200 / 191 / 56
\item Suspicious Tit For Tat: 176 / 185 / 160
\item Willing: 177 / 192 / 203
\item Remorseful Prober: 0.1: 178 / 168 / 114
\item First by Feld: 1.0, 0.5, 200: 179 / 145 / 84
\item First by Downing: 180 / 174 / 86
\item ZD-Mem2: 181 / 170 / 141
\item Worse and Worse 2: 182 / 142 / 98
\item Risky QLearner: 183 / 195 / 217
\item Cautious QLearner: 184 / 194 / 218
\item Arrogant QLearner: 185 / 196 / 216
\item Hesitant QLearner: 186 / 197 / 219
\item Detective: 187 / 189 / 166
\item Random Tit for Tat: 0.5: 188 / 188 / 180
\item First by Tullock: 189 / 160 / 116
\item k74r: 190 / 186 / 120 / 61
\item k54r: 191 / 191 / 143 / 58
\item Adaptive: 192 / 184 / 150
\item Worse and Worse: 193 / 190 / 212
\item Prober: 194 / 193 / 174
\item Hard Go By Majority: 5: 195 / 198 / 181
\item Hard Go By Majority: 196 / 202 / 194
\item Opposite Grudger: 197 / 208 / 236
\item Stochastic Cooperator: 198 / 187 / 187
\item Pun1: 199 / 206 / 199
\item Naive Prober: 0.1: 200 / 177 / 137
\item EasyGo: 201 / 220 / 259
\item First by Joss: 0.9: 202 / 176 / 136
\item ALLCorALLD: 203 / 211 / 228
\item Hard Go By Majority: 40: 204 / 201 / 188
\item Prober 4: 205 / 203 / 183
\item Prober 3: 206 / 199 / 175
\item Hard Go By Majority: 20: 207 / 207 / 185
\item Calculator: 208 / 182 / 135
\item Hard Go By Majority: 10: 209 / 209 / 186
\item SolutionB5: 210 / 210 / 184
\item Winner21: 211 / 221 / 225
\item Meta Mixer: 213 players: 212 / 205 / 195
\item Fortress3: 213 / 223 / 226
\item Fortress4: 214 / 224 / 222
\item Meta Hunter Aggressive: 7 players: 215 / 212 / 202
\item Cycler CCCCCD: 216 / 219 / 238
\item Stochastic WSLS: 0.05: 217 / 204 / 229
\item Cycler CCCDCD: 218 / 227 / 244
\item k71r: 219 / 222 / 220 / 60
\item Cycler CCCD: 220 / 228 / 245
\item ZD-SET-2: 0.25, 0.0, 2: 221 / 215 / 210
\item TF2: 222 / 229 / 231
\item Cooperator Hunter: 223 / 241 / 253
\item SelfSteem: 224 / 230 / 234
\item SolutionB1: 225 / 243 / 258
\item Cycler CCD: 226 / 231 / 239
\item Meta Winner Long Memory: 134 players: 227 / 216 / 189
\item Meta Winner: 213 players: 228 / 217 / 192
\item Alternator: 229 / 236 / 241
\item k63r: 230 / 240 / 248 / 57
\item Meta Winner Deterministic: 146 players: 231 / 218 / 190
\item ZD-Extort-2 v2: 0.125, 0.5, 1: 232 / 214 / 196
\item ZD-Extort-2: 0.1111111111111111, 0.5: 233 / 213 / 197
\item Meta Winner Ensemble: 213 players: 234 / 232 / 208
\item Meta Winner Stochastic: 67 players: 235 / 233 / 209
\item Win-Shift Lose-Stay: D: 236 / 244 / 247
\item Meta Winner Finite Memory: 79 players: 237 / 225 / 201
\item Cycler DC: 238 / 242 / 246
\item Meta Winner Memory One: 36 players: 239 / 234 / 207
\item k50r: 240 / 235 / 249 / 54
\item TF1: 241 / 238 / 224
\item ThueMorse: 242 / 250 / 256
\item Cycler DDC: 243 / 257 / 257
\item ZD-Extort3: 0.11538461538461539, 0.3333333333333333, 1: 244 / 226 / 213
\item AntiCycler: 245 / 259 / 263
\item Predator: 246 / 247 / 235
\item k36r: 247 / 251 / 243 / 63
\item ZD-Extort-4: 0.23529411764705882, 0.25, 1: 248 / 239 / 221
\item ThueMorseInverse: 249 / 248 / 251
\item CollectiveStrategy: 250 / 246 / 227
\item $\pi$: 251 / 260 / 264
\item UsuallyDefects: 252 / 249 / 237
\item Tricky Cooperator: 253 / 256 / 260
\item ZD-Mischief: 0.1, 0.0, 1: 254 / 237 / 223
\item Aggravater: 255 / 254 / 233
\item Better and Better: 256 / 258 / 242
\item ZD-Extortion: 0.2, 0.1, 1: 257 / 245 / 232
\item $e$: 258 / 261 / 265
\item First by Anonymous: 259 / 253 / 254
\item krandomc: 260 / 252 / 255 / 62
\item Bush Mosteller: 0.5, 0.5, 3.0, 0.5: 261 / 255 / 250
\item Desperate: 262 / 263 / 262
\item Gradual Killer: (D, D, D, D, D, C, C): 263 / 266 / 267
\item Meta Minority: 213 players: 264 / 268 / 268
\item Hopeless: 265 / 265 / 266
\item Bully: 266 / 269 / 269
\item Defector: 267 / 262 / 240
\item Handshake: 268 / 264 / 252
\item Tricky Defector: 269 / 267 / 261
\item $\phi$: 270 / 270 / 271
\item Negation: 271 / 271 / 270
\item Anti Tit For Tat: 272 / 272 / 272


==> assets/sp_tournament_full_rankings.tex <==
\begin{tabular}{lccccc}
\toprule
 & \makecell[c]{Mean Score} & \makecell[c]{Rank} & \makecell[c]{Mean\\Cooperation Rate} & \makecell[c]{Reproduced Mean\\Cooperation Rate} & \makecell[c]{S. and P. Mean\\Cooperation Rate} \\
\midrule
ZD-GTFT-2: 0.25, 0.5 & 2.834 & 1 & 0.926 & - & 0.855 \\
k42r & 2.825 & 2 & 0.903 & 0.916 & - \\
GTFT: 0.33 & 2.819 & 3 & 0.941 & - & 0.893 \\
k92r & 2.812 & 4 & 0.888 & 0.922 & 0.731 \\
k49r & 2.787 & 5 & 0.879 & 0.892 & - \\
k75r & 2.786 & 6 & 0.782 & 0.802 & - \\
k44r & 2.781 & 7 & 0.866 & 0.882 & - \\
k61r & 2.773 & 8 & 0.945 & 0.954 & - \\
k68r & 2.768 & 9 & 0.904 & 0.917 & - \\
k41r & 2.761 & 10 & 0.847 & 0.865 & - \\
k46r & 2.758 & 11 & 0.939 & 0.948 & - \\
k32r & 2.758 & 12 & 0.849 & 0.873 & - \\
k72r & 2.756 & 13 & 0.915 & 0.924 & - \\
k35r & 2.747 & 14 & 0.863 & 0.888 & - \\
k84r & 2.745 & 15 & 0.861 & 0.882 & - \\
k60r & 2.735 & 16 & 0.814 & 0.844 & - \\
k83r & 2.725 & 17 & 0.922 & 0.935 & - \\
k64r & 2.710 & 18 & 0.876 & 0.884 & - \\
k66r & 2.702 & 19 & 0.861 & 0.866 & - \\
Hard Tit For 2 Tats & 2.701 & 20 & 0.926 & - & 0.807 \\
k39r & 2.700 & 21 & 0.671 & 0.676 & - \\
k47r & 2.696 & 22 & 0.709 & 0.723 & - \\
k58r & 2.694 & 23 & 0.846 & 0.852 & - \\
k31r & 2.690 & 24 & 0.908 & 0.920 & - \\
k88r & 2.684 & 25 & 0.851 & 0.861 & - \\
k79r & 2.678 & 26 & 0.864 & 0.875 & - \\
k90r & 2.676 & 27 & 0.943 & 0.964 & 0.844 \\
k67r & 2.676 & 28 & 0.743 & 0.749 & - \\
k91r & 2.662 & 29 & 0.889 & 0.873 & - \\
k51r & 2.646 & 30 & 0.892 & 0.905 & - \\
k80r & 2.641 & 31 & 0.813 & 0.809 & - \\
k43r & 2.641 & 32 & 0.673 & 0.666 & - \\
k86r & 2.639 & 33 & 0.803 & 0.811 & - \\
k38r & 2.639 & 34 & 0.865 & 0.874 & - \\
k59r & 2.635 & 35 & 0.889 & 0.891 & - \\
k56r & 2.635 & 36 & 0.890 & 0.891 & - \\
k78r & 2.634 & 37 & 0.720 & 0.755 & - \\
k40r & 2.625 & 38 & 0.742 & 0.746 & - \\
k55r & 2.620 & 39 & 0.903 & 0.903 & - \\
k57r & 2.620 & 40 & 0.799 & 0.811 & - \\
k70r & 2.596 & 41 & 0.752 & 0.769 & - \\
k73r & 2.595 & 42 & 0.761 & 0.764 & - \\
k69r & 2.591 & 43 & 0.672 & 0.702 & - \\
k37r & 2.590 & 44 & 0.778 & 0.791 & - \\
k81r & 2.589 & 45 & 0.774 & 0.779 & - \\
k87r & 2.586 & 46 & 0.760 & 0.766 & - \\
k85r & 2.584 & 47 & 0.713 & 0.726 & - \\
k76r & 2.576 & 48 & 0.636 & 0.680 & - \\
k53r & 2.568 & 49 & 0.730 & 0.728 & - \\
k65r & 2.559 & 50 & 0.718 & 0.715 & - \\
k52r & 2.545 & 51 & 0.820 & 0.838 & - \\
Win-Stay Lose-Shift & 2.544 & 52 & 0.809 & - & 0.808 \\
Hard Tit For Tat & 2.539 & 53 & 0.710 & - & 0.663 \\
Cooperator & 2.522 & 54 & 1.000 & - & 1.000 \\
k45r & 2.521 & 55 & 0.726 & 0.754 & - \\
k82r & 2.491 & 56 & 0.529 & 0.544 & - \\
k62r & 2.490 & 57 & 0.732 & 0.754 & - \\
k34r & 2.478 & 58 & 0.647 & 0.652 & 0.655 \\
Hard Go By Majority & 2.375 & 59 & 0.658 & - & 0.459 \\
k48r & 2.300 & 60 & 0.504 & 0.499 & - \\
First by Joss: 0.9 & 2.280 & 61 & 0.501 & - & 0.345 \\
k50r & 2.248 & 62 & 0.929 & 0.930 & - \\
k89r & 2.212 & 63 & 0.504 & 0.498 & - \\
k77r & 2.165 & 64 & 0.327 & 0.332 & - \\
k54r & 2.118 & 65 & 0.483 & 0.467 & - \\
k33r & 2.108 & 66 & 0.424 & 0.411 & - \\
k63r & 2.096 & 67 & 0.502 & 0.502 & - \\
k71r & 2.032 & 68 & 0.166 & 0.158 & - \\
k74r & 1.881 & 69 & 0.171 & 0.174 & - \\
ZD-Extort-2: 0.1111111111111111, 0.5 & 1.838 & 70 & 0.254 & - & 0.232 \\
krandomc & 1.698 & 71 & 0.500 & 0.500 & 0.500 \\
k36r & 1.520 & 72 & 0.092 & 0.092 & - \\
Defector & 1.472 & 73 & 0.000 & - & 0.000 \\
\bottomrule
\end{tabular}


==> assets/sp_tournament_overall_cooperation_rate.tex <==
0.732

==> assets/sp_tournament_rankings.tex <==
\begin{tabular}{lrrrrr}
\toprule
 & Mean Score & Rank & Mean Cooperation Rate & Reproduced Mean Cooperation Rate & S. and P. Mean Cooperation Rate \\
Name &  &  &  &  &  \\
\midrule
ZD-GTFT-2: 0.25, 0.5 & 2.834 & 1 & 0.926 & NaN & 0.855 \\
k42r & 2.825 & 2 & 0.903 & 0.916 & NaN \\
GTFT: 0.33 & 2.819 & 3 & 0.941 & NaN & 0.893 \\
k92r & 2.812 & 4 & 0.888 & 0.922 & 0.731 \\
k49r & 2.787 & 5 & 0.879 & 0.892 & NaN \\
k75r & 2.786 & 6 & 0.782 & 0.802 & NaN \\
k44r & 2.781 & 7 & 0.866 & 0.882 & NaN \\
k61r & 2.773 & 8 & 0.945 & 0.954 & NaN \\
k68r & 2.768 & 9 & 0.904 & 0.917 & NaN \\
k41r & 2.761 & 10 & 0.847 & 0.865 & NaN \\
k46r & 2.758 & 11 & 0.939 & 0.948 & NaN \\
k32r & 2.758 & 12 & 0.849 & 0.873 & NaN \\
k72r & 2.756 & 13 & 0.915 & 0.924 & NaN \\
k35r & 2.747 & 14 & 0.863 & 0.888 & NaN \\
k84r & 2.745 & 15 & 0.861 & 0.882 & NaN \\
k60r & 2.735 & 16 & 0.814 & 0.844 & NaN \\
k83r & 2.725 & 17 & 0.922 & 0.935 & NaN \\
k64r & 2.710 & 18 & 0.876 & 0.884 & NaN \\
k66r & 2.702 & 19 & 0.861 & 0.866 & NaN \\
Hard Tit For 2 Tats & 2.701 & 20 & 0.926 & NaN & 0.807 \\
k39r & 2.700 & 21 & 0.671 & 0.676 & NaN \\
k47r & 2.696 & 22 & 0.709 & 0.723 & NaN \\
k58r & 2.694 & 23 & 0.846 & 0.852 & NaN \\
k31r & 2.690 & 24 & 0.908 & 0.920 & NaN \\
k88r & 2.684 & 25 & 0.851 & 0.861 & NaN \\
\bottomrule
\end{tabular}

